On Efficient Approximate Queries over Machine Learning Models

The question of answering queries over ML predictions has been gaining attention in the database community. This question is challenging because the cost of finding high quality answers corresponds to invoking an oracle such as a human expert or an expensive deep neural network model on every single item in the DB and then applying the query. We develop a novel unified framework for approximate query answering by leveraging a proxy to minimize the oracle usage of finding high quality answers for both Precision-Target (PT) and Recall-Target (RT) queries. Our framework uses a judicious combination of invoking the expensive oracle on data samples and applying the cheap proxy on the objects in the DB. It relies on two assumptions. Under the Proxy Quality assumption, proxy quality can be quantified in a probabilistic manner w.r.t. the oracle. This allows us to develop two algorithms: PQA that efficiently finds high quality answers with high probability and no oracle calls, and PQE, a heuristic extension that achieves empirically good performance with a small number of oracle calls. Alternatively, under the Core Set Closure assumption, we develop two algorithms: CSC that efficiently returns high quality answers with high probability and minimal oracle usage, and CSE, which extends it to more general settings. Our extensive experiments on five real-world datasets on both query types, PT and RT, demonstrate that our algorithms outperform the state-of-the-art and achieve high result quality with provable statistical guarantees.

==> algorithms_backup.tex <==
\section{Algorithms}
\label{sec:algos}
%We now describe our solutions, given the assumptions stated in \S~\ref{sec:approach}.

\subsection{Algorithms Based on Proxy Quality}
\label{subsec:alg_pq} 
We formally state the {\sc Proxy Quality} assumption (\S~\ref{subsubsec:proxy_assump}) and show how the success probability of a set $S \subset D$ can be computed (\S~\ref{subsubsec:subset_success}). Then, we explore monotonicity of success probability and expected CR (\S~\ref{subsubsec:subset_compare}) to prune out unpromising solutions and efficiently find optimal answers. Algorithms \pqa and \pqe, based on this assumption, are given in \S~\ref{subsubsec:alg_pqa_pqe}. 

\eat{ 
We study how to find valid answers w.h.p. to a query with \textbf{zero} oracle calls and maximal expected CR under \textsc{Proxy Quality} (\S~\ref{sec:approach}). 
We develop our solutions by answering the following questions in order, (i) \textit{How to validate the success probability for any $S\subseteq D$ and a query (\S~\ref{subsubsec:subset_success})?}  (ii) \textit{How to compare success probability and expected CR for any subset of $D$ w.r.t. a query (\S~\ref{subsubsec:subset_compare})?} At the end, in \S \ref{subsubsec:alg_pqa_pqe}, we develop our algorithms to efficiently find the optimal answer $Ans \subseteq D$ for a query with maximal expected CR $\mathbb{E}[\measurecomp(Ans)]$ and high success probability $\pos(Ans, \measure, \gamma) \geq 1 - \delta$ with zero oracle calls. 
} 

% In \S~\ref{subsubsec:subset_success}, we show how to compute success probability $\pos(S, M, \gamma)$ for any $S\subseteq D$ and a query. In \S~\ref{subsubsec:subset_compare}, we prove monotonicity relations to efficiently compare success probability and expected CR for any subset of $D$ w.r.t. a query. In \S \ref{subsubsec:alg_pqa_pqe}, we develop our algorithms to efficiently find the optimal answer $Ans \subseteq D$ for a query with maximal $\mathbb{E}[\measurecomp(Ans)]$ and $\pos(Ans, \measure, \gamma) \geq 1 - \delta$ with zero oracle calls. 

\subsubsection{Proxy Quality Assumption}
\label{subsubsec:proxy_assump}
The assumption says that given a query, the deviations between the proxy distance and oracle distance of different objects $x_i\in D$ are i.i.d. random variables: for  $x_i \in D, dist^\oracle(x_i) = dist^\proxy(x_i) + \epsilon_i$, where 
$\epsilon_i$ are i.i.d., $\epsilon_i \sim \mathcal{X}$.

\eat{ 
\textsc{Proxy Quality} quantifies proxy quality w.r.t. oracle in a probabilistic manner. The assumption says that, given a query, the difference between oracle distance $dist^O(x_i)$ and proxy distance $dist^P(x_i)$ for $x_i \in D$ are i.i.d. random variables. 
Formally,
\begin{assumption} [Proxy Quality Assumption]
\label{assump:proxy_quality_assumption}
\begin{small}
\begin{equation}
\forall x_i \in D, dist^\oracle(x_i) = dist^\proxy(x_i) + \epsilon_i
\end{equation}
\end{small}
where $\epsilon_i$ are i.i.d., $\epsilon_i \sim \mathcal{X}$. 
\end{assumption}
} 


Under this assumption,
we have the oracle distance distribution for any $x_i \in D$,  after observing the proxy distance. 
The probability of $x_i \in D$  being an oracle neighbor is given by:
\begin{small}
\begin{equation}
\label{fact:identity}
\begin{split}
Pr[x_i \in \nearneighbor]&=Pr[dist^\oracle(x_i) \leq r] =Pr[\epsilon_i \leq r-dist^\proxy(x_i)]
\end{split}
\end{equation}
\end{small}
The RHS of Eq. \ref{fact:identity} is the cdf of $\epsilon_i \sim \mathcal{X}$ evaluated at $r-dist^\proxy(x_i)$, i.e., $CDF_{\mathcal{X}}(r-dist^\proxy(x_i))$. For simplicity,  define $\phi(x_i) := CDF_{\mathcal{X}}(r-dist^\proxy(x_i))$ and $\Phi(D)=\{\phi(x_i) \mid x_i \in D\}$. 
%Clearly, $\phi(x_i) \geq \phi(x_j)$ if $dist^P(x_i) \leq dist^P(x_j)$ for $x_i, x_j \in D$. 
%\hl{Given a query with failure rate} $\delta$, \hl{we further assume} $\max \{\phi(x_i) \mid x_i \in D\} \geq 1 - \delta$ \hl{to ensure the proxy does not deviate from oracle too much.} 
%Given a dataset $D$, we define an index function $\indexphi: D \to \{i \mid 1\leq i \leq |D|\}$ mapping objects $x_i\in D$ to a decreasing order w.r.t. $\phi(x_i)$. Specifically, $\forall x_i, x_j \in D$, $\indexphi(x_i) \leq \indexphi(x_j)$ if $\phi(x_i) \geq \phi(x_j)$.
%
$\phi(x_i)$ provides the probability that $x_i$ is an oracle neighbor. Next,
we seek the likelihood of any $S \subseteq D$ containing a certain number of oracle neighbors, in order to  compute the success probability of $S$.

Recall that for any subset $S \subseteq D$, $N_S = |S \cap \nearneighbor|$  is the number of oracle neighbors in $S$.  
%Given $S \subseteq D$ and $\Phi(S)$, 
$N_S$ is thus a random variable equal to the sum of $|S|$ independent Bernoulli trials, %\cite{bernoulli1713ars}, 
each of which has a success probability $\phi_i \in \Phi(S)$. 
Let $p_{N_S}(k) := Pr[N_S = k]$ be the probability mass function for any $S \subseteq D$ and $0\leq k \leq |S|$. We  show how to compute it efficiently.


% By definition, $N_S$ is a Poisson binomial random variable \cite{fernandez2010poisson}, after observing proxy distance for each $x_i \in S$ under Assumption \ref{assump:proxy_quality_assumption}.
% We use a \textit{direct convolution} method \cite{osti_1548776} to compute the probability distribution of $N_S$ for any $S \subseteq D$. We define $p_{N_S}(k) = Pr[N_S = k]$ for any $S \subseteq D$ and integer $k$.

An important fact is that, given $S \subseteq D$, $x_i \notin S$, $p_{N_{S\cup \{x_i\}}}$ and $p_{N_{S}}$ have the following recurrence relation,
\begin{small}
\begin{equation}
\label{eq:pndist_update}
\begin{split}
    p_{N_{S\cup \{x_i\}}}(k)=p_{N_{S}}(k-1)\cdot \phi(x_i) + p_{N_{S}}(k)\cdot (1-\phi(x_i))\\
\end{split}
\end{equation}
\end{small}
for $0\leq k \leq |S|+1$.
Eq. \ref{eq:pndist_update} says how to compute the probability mass function $p_{N_{S\cup \{x_i\}}}$ from $p_{N_{S}}$, for any $S \subseteq D$ and $x_i \notin S$. This recurrence relation directly suggests a way to compute $p_{N_{S}}$ for any $S$ with incremental updates, called  \textit{direct convolution} \cite{osti_1548776}.
% We can start from $S=\varnothing$ and apply Equation \ref{eq:pndist_update} recursively to compute $p_{N_{S}}$ for any $S \subseteq D$.
The algorithm is given in Algorithm~\ref{alg:compute_pndist}.
\normalem
\begin{algorithm}
\caption{Compute $p_{N_S}$}
\label{alg:compute_pndist}
\DontPrintSemicolon
  \SetKwFunction{fpns}{pNs}
  \SetKwFunction{fpnsupdate}{pNsUpdate}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\fpns{$\Phi_S=\Phi(S)$}}{
    $p_{N_S}[0] \gets 1$\; \label{pbdist:init}
    \For{$i \gets 1, 2, \cdots, |S|$\label{pbdist:convl_s}}{
    $p_{N_S} \gets $ \fpnsupdate{$p_{N_S}$, $\Phi_S[i]$, $i$}\label{pbdist:convl_e}
    }
    \KwRet $p_{N_S}$
  }
  \Fn{\fpnsupdate{$p_{N_S}$, $\phi_i$, $i$}}{
    \For{$j \gets 0, 1, \cdots, i$ \label{pbdist:update_s}}{
            $p_{N_S}[j] \gets p_{N_S}[j-1]\phi_i + p_{N_S}[j](1-\phi_{i})$\label{pbdist:update_e}}
    \KwRet $p_{N_S}$
    }
\end{algorithm}
\ULforem

$p_{N_S}$ is implemented by an array. In line \ref{pbdist:init}, we initialize the array $p_{N_S}[0]=1$. In lines \ref{pbdist:convl_s}-\ref{pbdist:convl_e}, we iteratively update $p_{N_S}$ by including $x_i \in S$, $1\leq i \leq |S|$,  in any order. The distribution updates, described in lines \ref{pbdist:update_s}-\ref{pbdist:update_e}, are a direct implementation of Eq. \ref{eq:pndist_update}.

\subsubsection{Computing $\pos(S,\measure,\gamma)$}
\label{subsubsec:subset_success}
\eat{We have seen how to compute the probability distribution function $p_{N_S}$ for any $S \subseteq D$. We now discuss how to use $p_{N_S}$ to compute the probability for any $S \subseteq D$ being a valid answer to a given PT or RT query, i.e, $\pos(S,\precis,\gamma)$ and $\pos(S,\recall,\gamma)$.} 
We next discuss how to use $p_{N_S}$ to compute $\pos(S,\measure,\gamma)$, the success probability for $S$ to be a valid answer. We have the following fact, where $\overline{S} := D \setminus S$:
\begin{fact}
\label{fact:pos_pqa}
Given $S \subseteq D$ and $\gamma \in (0,1)$, 
\vspace*{-2ex} 
\begin{small}
\begin{equation}
\label{eq:precis_prob}
\begin{split}
    \pos(S, \precis, \gamma) &= Pr[\frac{N_S}{|S|} \geq \gamma]
    =\sum_{k=\lceil |S|\gamma \rceil}^{|S|}p_{N_S}(k)\\
\end{split}
\end{equation}
\end{small}
\vspace*{-1.5ex} 
\begin{small}
\begin{equation}
\label{eq:recall_prob}
\begin{split}
    \pos(S, \recall, \gamma) &= Pr[\frac{N_S}{|\nearneighbor|} \geq \gamma]
    =\sum_{j=0}^{|S|} p_{N_S}(j) \sum_{k=0}^{\lfloor j (1-\gamma)/\gamma \rfloor} p_{N_{\overline{S}}}(k)\\
\end{split}
\end{equation}
\end{small}
\end{fact}

For PT queries, the precision of $S \subseteq D$ goes up as $S$ contains more oracle neighbors.  
The probability of $S$ having a precision no less than $\gamma$ equals the probability of $S$ containing at least $|S|\gamma$ oracle neighbors, i.e., $Pr[N_S \geq |S|\gamma]$.
Eq. \ref{eq:precis_prob} lets us compute this probability.

For RT queries, the recall of $S \subseteq D$ goes up as $S$ contains more oracle neighbors \textit{relative to} the complement $\overline{S} = D \setminus S$: 
if $S$ contains $0 \leq j \leq |S|$ oracle neighbors, the conditional probability of $S$ having a recall no less than $\gamma$ equals  the probability that $\overline{S}$ contains no more than $j (1-\gamma)/\gamma$ oracle neighbors, i.e., $Pr[N_{\overline{S}} \leq j (1-\gamma)/\gamma]$. 
By the law of total probability \cite{Grimmett1986-GRIPAI}, the overall success probability $\pos(S, \recall, \gamma)$ equals  the summation of the product between the conditional success probability, $Pr[N_{\overline{S}} \leq j (1-\gamma)/\gamma]$, and the marginal probability, $Pr[N_S=j]$,  $0\leq j \leq |S|$. 
Using Eq. \ref{eq:recall_prob}, we use $p_{N_{S}}$ and $p_{N_{\overline{S}}}$ to compute this probability.

% Given $S \subseteq D$, for PT queries, $\pos(S, \precis, \gamma)$ equals to the probability of $N_S$ being no less than $|S|\gamma$, as described in Equation \ref{eq:precis_prob}. For RT queries, if $N_S=j$ for $0\leq j \leq |S|$, the conditional success probability equals to the likelihood for $N_{D \setminus S}$ being no larger than $\frac{(1-\gamma)j}{\gamma}$. The overall success probability $\pos(S, M_r, \gamma)$, therefore, equals to the summation of the product between the conditional success probability and the probability of each condition, that is, $p_{N_S}(j)$ for $0\leq j \leq |S|$. This relation is given in Equation \ref{eq:recall_prob}.  

Fact \ref{fact:pos_pqa} directly suggests Algorithm \ref{alg:subset_success}, which computes $\pos(S,M,\gamma)$ for any $S \subseteq D$ for a given query. Lines \ref{fpospt:s}-\ref{fpospt:e} are a direct implementation of Eq. \ref{eq:precis_prob}, while lines \ref{fposrt:s}-\ref{fposrt:e} apply Eq. \ref{eq:recall_prob} iteratively.
\normalem
\begin{algorithm}
\caption{Compute $\pos(S,M,\gamma)$}
\label{alg:subset_success}

\DontPrintSemicolon
  \SetKwFunction{fprecis}{PoS-Mp}
  \SetKwFunction{frecall}{PoS-Mr}
  \SetKwProg{Fn}{Function}{:}{}
  \SetKwFunction{Sum}{Sum}
  
\Fn{\fprecis{$p_{N_S}$, $\gamma$}\label{fpospt:s}}
{
\KwRet \Sum{$\{p_{N_S}[k] \mid \lceil |S|\gamma \rceil \leq k \leq |S|\}$}\;
\label{fpospt:e}}

\Fn{\frecall{$p_{N_S}$, $p_{N_{\overline{S}}}$, $\gamma$}\label{fposrt:s}}
{
$prob \gets 0$\;
\For{$j\gets 0, 1, \cdots, |S|$}{
$prob \gets prob + p_{N_S}[j] \cdot $ \Sum{$\{ p_{N_{\overline{S}}}[k] \mid 0\leq k \leq \lfloor j (1-\gamma)/\gamma \rfloor \}$}\;
}
\KwRet $prob$\;
\label{fposrt:e}}
\end{algorithm}
\ULforem



\subsubsection{$\pos(S,M,\gamma)$ \& $\mathbb{E}(\measurecomp(S))$ Monotonicity}
\label{subsubsec:subset_compare}

We have seen how to compute success probability for any $S \subseteq D$. Next, we are interested in the monotonicity of success probability and expected CR between any subsets of $D$ to efficiently filter out unpromising solutions. For $S \subseteq D$, we are interested in two operations to generate new answers: (i) replace $x_i \in S$ with $x_j \notin S$, and (ii) append $S$ with a new object $x \notin S$.

% $\pos(S,M,\gamma)$ and $\pos(S',M,\gamma)$ for any subsets $S,S' \subseteq D$. Moreover, we would like to efficiently compare the expected complementary rates, that is, $\mathbb{E}(\measurecomp(S))$ and $\mathbb{E}(\measurecomp(S'))$, for any subsets $S,S' \subseteq D$.

We first give the monotonicity relation of success probability $\pos(S,M,\gamma)$ and expected CR $\mathbb{E}(\measurecomp(S))$ for any $S \subseteq D$, under replacement operation.
\begin{lemma} [Monotonicity of Replacement]
\label{lemma:monoto_replace}
Given $x_i \in S \subseteq D$, $x_j \notin S$, denote $S'=S \cup \{x_j\} \setminus \{x_i\}$. $\forall \gamma \in (0,1)$, if $\phi(x_i) \leq \phi(x_j)$, we have
\begin{small}
\begin{equation}
\begin{split}
     \pos(S, M, \gamma) &\leq \pos(S', M, \gamma)\hspace{0.5cm}
\mathbb{E}[\measurecomp(S)] \leq \mathbb{E}[\measurecomp(S')]\\
\end{split}
\end{equation}
\end{small}
\end{lemma}
Proof of Lemma \ref{lemma:monoto_replace} relies on the notion \textit{usual stochastic order} \cite{Nair2013}. Due to space limitation, we leave all the proofs to a complete version of this paper.

Lemma \ref{lemma:monoto_replace} says that, given $S \subseteq D$, if we replace $x_i \in S$ with $x_j \notin S$, where $x_j$ is more likely to be an oracle neighbor, both the success probability and the expected CR of $S$ will monotonically increase, for a given query.
Lemma \ref{lemma:monoto_replace} can be used to prune out a majority of unpromising solutions in the early stage of query processing. Specifically, given a query, we show that any $S \subseteq D$ except $\topphi{k}$ for $1\leq k \leq |D|$ can be excluded from consideration as optimal answers. Recall $\topproxy{k}$ is the $k$ nearest neighbors of the query object w.r.t. the proxy distance. 
%We show that $\topphi{k}$ maximizes the success probability and expected CR within all subsets $S \subseteq D$ of $|S|=k$, for $1\leq k \leq |D|$. 
Formally,
\begin{theorem}
\label{theorem:topk}
$\forall \gamma \in (0,1)$, $\forall 1\leq k \leq |D|$,
\begin{small}
\begin{equation}
\begin{split}
    \topphi{k} &\in \argmax_{S\subseteq D, |S|=k} \pos(S, M, \gamma) \hspace{0.5cm}
    \topphi{k} \in \argmax_{S\subseteq D, |S|=k} \mathbb{E}[\measurecomp(S)]
\end{split}
\end{equation}
\end{small}
\end{theorem}

Theorem \ref{theorem:topk} entails that, given a query, the optimal answer must be $\topphi{k^*}$ for some $1\leq k^* \leq |D|$. The next question is how to efficiently find the $\topphi{k^*}$. We study the append operation and have the following monotonicity relations,
\begin{lemma} [Monotonicity of Append]
\label{lemma:monoto_append}
$\forall \gamma \in (0,1)$, $\forall 1\leq k \leq |D|-1$,
\begin{small}
\begin{equation}
\begin{split}
\pos(\topphi{k}, M_r, \gamma) &\leq \pos(\topphi{k+1}, M_r, \gamma)\hspace{0.2cm}
\mathbb{E}[\recall(\topphi{k})] \leq \mathbb{E}[\recall(\topphi{k+1})]
\end{split}
\end{equation}
\end{small}
\end{lemma}

Lemma \ref{lemma:monoto_append} states that by increasing $k$ both the probability of $\topkproxy{k}$ having a high recall and the expected recall of $\topkproxy{k}$ will monotonically increase.
In other words,
the success probability of $\topphi{k}$ monotonically increases for RT queries, and the expected CR of $\topphi{k}$ monotonically increases for PT queries, as $k$ increases. Lemma \ref{lemma:monoto_append} can be used to filter out unpromising solutions and supports efficient search for $\topphi{k^*}$.

% In the next subsection, we are going to show how to develop efficient algorithms with Lemma \ref{lemma:monoto_append}.

\subsubsection{\pqa \& \pqe}
\label{subsubsec:alg_pqa_pqe}

In this subsection, we develop our algorithm \pqa and \pqe with Lemma \ref{lemma:monoto_append}. Given a query, \pqa uses zero oracle call to return high probability valid answers with maximal expected CR under \textsc{Proxy Quality} assumption. \pqe calibrates \pqa with good heuristics and applies in general settings.

We are going to first present \pqa. Recall that Lemma \ref{lemma:monoto_append} states the monotonicity of expected CR for PT queries, and success probability for RT queries. \pqa employs these two monotonicity relations to filter out a majority of unpromising solutions and return the optimal answer efficiently. 

For PT queries, \pqa computes the largest $k$ of $\pos(\topphi{k}, \precis, \gamma) \geq 1 - \delta$, for $1\leq k \leq |D|$, denoted as $k^*$. By Lemma \ref{lemma:monoto_append}, $\topphi{k^*}$ is the optimal answer which gives the maximal expected CR.
Recall that $\pos(S, \precis, \gamma)$ can be derived from $p_{N_S}$ in linear time (see Algorithm \ref{alg:subset_success}), and $p_{N_S}$ can be computed from $p_{N_{S \setminus \{x_i\}}}$ in linear time (see Algorithm \ref{alg:compute_pndist}), for any $x_i \in S \subseteq D$. \pqa-PT incrementally computes $p_{N_{D_k}}$ for each $1 \leq k \leq |D|$ and $\pos(\topphi{k}, \precis, \gamma)$ accordingly.
At the end, \pqa returns $\topphi{k^*}$ where $k^* = \max\{1\leq k \leq |D| \mid \pos(\topphi{k}, M_p, \gamma) \geq 1 - \delta \}$. 

For RT queries, given the monotonicity of the success probability as claimed by Lemma \ref{lemma:monoto_append}, \pqa-RT use binary search to identify the smallest $k =\underline{k}$ such that  $\pos(\topkproxy{k}, \measure, \gamma) \geq 1-\delta$. Next, \pqa-RT computes the expected CR of $\topphi{k}$ for each $\underline{k} \leq k \leq |D|$, and returns $\topphi{k^*}$ where $k^*=\argmax_{ \underline{k} \leq k \leq |D|} \mathbb{E}[\precis(\topphi{k})]$.

The algorithm is presented in Algorithm \ref{alg:pqa}.\pqa-PT is given in lines \ref{pqapt:s} to \ref{pqapt:e}. In lines \ref{pqapt:comp_pns_s} to \ref{pqapt:comp_pns_e}, we incrementally compute the $p_{N_{\topphi{k}}}$ for $1\leq k \leq |D|$. In line \ref{pqapt:find_kmax_s} to \ref{pqapt:e}, we keep tracking the largest $k=k^*$ of $\pos(\topphi{k}, \precis, \gamma) \geq 1 - \delta$ for $1\leq k \leq |D|$, and return $\topphi{k^*}$ as the answer. The overall time complexity is $O(|D|^2)$.
\normalem
\begin{algorithm} 
\caption{PQA}
\label{alg:pqa}

\DontPrintSemicolon
  \SetKwFunction{pqapt}{PQA-PT}
  \SetKwProg{Fn}{Function}{:}{}
%   \SetKwFunction{fprecis}{PoS-Mp}

  \SetKwFunction{pqart}{PQA-RT}
%   \SetKwFunction{frecall}{PoS-Mr}
%   \SetKwFunction{func}{pNs}
%   \SetKwFunction{Sum}{Sum}
  
\Fn{\pqapt{$\Phi_D=\Phi(D)$, $\gamma$, $\delta$} \label{pqapt:s}}
{$p_{N_S}[0] \gets 1$\; \label{pqapt:comp_pns_s}
\For{$i \gets 1, 2, \cdots, |D|$}{
    $p_{N_S} \gets $ \fpnsupdate{$p_{N_S}$, $\Phi_D[i]$, $i$}\; \label{pqapt:comp_pns_e}
    \If{\fprecis{$p_{N_S}$, $\gamma$} $\geq 1-\delta$ \label{pqapt:find_kmax_s}}
    {$k^* \gets i$}}
\KwRet $\topphi{k^*}$
\label{pqapt:e}}
  
\Fn{\pqart{$\Phi_D=\Phi(D)$, $\gamma$, $\delta$} \label{pqart:s} }
{
$\underline{k} \gets 1$; $\overline{k} \gets |D|$\;\label{pqart:bs_s}
\While {$\underline{k} < \overline{k}$}{
$mid \gets \lfloor (\underline{k} + \overline{k}) / 2 \rfloor$\;
$p_{N_S} \gets$ \fpns{$\Phi(S)$};\ $p_{N_{\overline{S}}} \gets$ \fpns{$\Phi(\overline{S})$}\;
\eIf{\frecall{$p_{N_S}$, $p_{N_{\overline{S}}}$, $\gamma$} $< 1-\delta$}
{$\underline{k} \gets mid+1$}
{$\overline{k} \gets mid$}
}\label{pqart:bs_e}

$p_{N_S} \gets $ \fpns{$\Phi(\topphi{\underline{k}})$}\;
$E\measurecomp \gets \label{pqart:maxexp_s}$ \Sum{$\{p_{N_S}[i]\cdot i / {\underline{k}} \mid 1 \leq i \leq \underline{k}\}$} \tcc*{Expected precision of $S$}
\For{$i \gets \underline{k}+1, \underline{k}+2, \cdots, |D|$}{
$p_{N_S} \gets $ \fpnsupdate{$p_{N_S}$, $\Phi_D[i]$, $i$}\;
    $E\measurecomp' \gets $ \Sum{$\{p_{N_S}[j]\cdot j / {i} \mid 1 \leq j \leq i\}$}\;
    \If{$E\measurecomp' > E\measure$}{
    $E\measure \gets E\measurecomp'$;
    $k^* \gets i$\;}
}
\KwRet $\topphi{k^*}$
\label{pqart:e}}

\end{algorithm}
\ULforem



\pqa-RT is given in line \ref{pqart:s} to \ref{pqart:e}. In line \ref{pqart:bs_s} to \ref{pqart:bs_e}, we use binary search to find the smallest $k=\underline{k}$ of $\pos(\topphi{k}, \recall, \gamma) \geq 1 - \delta$. Next, in line \ref{pqart:maxexp_s} to \ref{pqart:e}, we compute $\mathbb{E}[\precis(\topphi{k})]$ for each $\underline{k} \leq k \leq |D|$ and return $\topphi{k^*}$ of the maximal expected CR. 
The overall time complexity is dominated by binary search and, therefore, is $O(log(|D|)|D|^2)$. 
% We realize that there exists an $O(|D|^2)$ implementation to \pqa-RT, which computes $p_{N_S}$ and $p_{N_{D \setminus S}}$ recursively instead of computing it from scratch at each call. However, we test it in practice and find it numerically unstable. We leave to future work how to stabilize this quadratic time complexity implementation.

Notice that \pqa requires $\Phi(D)$ as the input for a given query, which is often challenging to obtain as a prior.
In \pqe, we employ $\epsilon_i \sim \mathcal{N}(\mu, \sigma)$ for all $x_i \in D$ according to our data analysis, and present a heuristic strategy to compute $\Phi(D)$ for a given query. 
$\mathcal{N}(\mu, \sigma)$ is a normal distribution of mean $\mu$ and standard deviation $\sigma$. We want to choose $\mu$ and $\sigma$ with good heuristics.
For $\mu$, since proxy approximates the oracle and is believed as an unbiased estimator, we empirically choose $\mu=0$. For $\sigma$, given a budget $b$, \pqe samples and probes $b$ objects to estimate $\sigma$ as $\hat{\sigma}$. 
% Since \textsc{Proxy Quality} assumption may not hold in general, 
We further introduce a hyper-parameter $\sigma_0$ to account for the deviation from our assumption. In the ideal case where \textsc{Proxy Quality} assumption holds, $\sigma_0=0$.  We heuristically set $\sigma = \hat{\sigma} + \sigma_0$. We use $\mathcal{N}(\mu, \sigma)$ to compute $\Phi(D)$ and pass it to \pqa to find answers to a given query.
\normalem
\begin{algorithm}
\caption{PQE}
\label{alg:pqe}

\DontPrintSemicolon
  \SetKwFunction{fpqe}{PQE}
  \SetKwProg{Fn}{Function}{:}{}
%   \SetKwFunction{fpqapt}{PQA-PT}
%   \SetKwFunction{fpqart}{PQA-RT}
  \SetKwFunction{sample}{Sample}
  \SetKwFunction{std}{std}
  \SetKwFunction{cdf}{CDF$_{N(0, \sigma)}$}
  
\Fn{\fpqe{$D$, $\gamma$, $\delta$, $r$, $b$, $\sigma_0$}}
{
$S \gets$ \sample{$D$, $b$}\; \label{pqe:est_s}
$\sigma \gets \sigma_0 + $ \std{$\{ dist^O(x) - dist^P(x)\mid x \in S\}$}\; 
$\Phi_D \gets \{$ \cdf{$r - dist^P(x)$} $\mid x \in D\}$\; \label{pqe:est_e}
\eIf{RT query \label{pqe:pqa_s}}
{\KwRet \pqart{$\Phi_D$, $\gamma$, $\delta$}}
{\KwRet \pqapt{$\Phi_D$, $\gamma$, $\delta$}\label{pqe:pqa_e}}
}
\end{algorithm}
\ULforem

Algorithm \ref{alg:pqe} contains the steps.
In lines \ref{pqe:est_s} to \ref{pqe:est_e}, we draw a sample $S \subseteq D$ of $|S|=b$ to estimate $\sigma$ and compute $\Phi(D)$. In line \ref{pqe:pqa_s} to \ref{pqe:pqa_e}, we invoke \pqa algorithms with $\Phi(D)$ for PT or RT queries. The time complexity in addition to \pqa algorithms is $O(|D|)$.

By design, \pqa ensures that the returned answer $Ans \subseteq D$ satisfies success probability constraint with maximal expected CR at zero oracle call, under \textsc{Proxy Quality} assumption. \pqe is a heuristic extension to \pqa which finds empirically good answers in general settings. 

In situations where proxy quality is hard to quantify, we introduce \textsc{Core Set Closure} assumption and develop two efficient algorithms $\csa$ and $\cse$, as presented in the next subsection.

\subsection{Algorithms under Core Set Closure}
\label{subsec:alg_cs}
%We are now interested in how to find valid answers w.h.p. to a given query with a minimal oracle usage.

We formally introduce the {\sc Core Set Closure} assumption in \S~\ref{subsubsec:csa_assumption}.
Under this assumption, we develop algorithms \csa in \S~\ref{subsubsec:csa} and \cse in \S~\ref{subsubsec:cse} to find high probability valid answers to any given query with a minimal expected number of oracle calls.

\subsubsection{Core Set Closure}
\label{subsubsec:csa_assumption}
% Given a dataset $D$, define an index function $\indexproxy: D \to \{i \mid 1\leq i \leq |D|\}$ mapping objects to an increasing order w.r.t. proxy distance. Specifically, $\forall x_i, x_j \in D$, $\indexproxy(x_i) \leq \indexproxy(x_j)$ if $dist^P(x_i) \leq dist^P(x_j)$. Denote $\topproxy{k} = \{x \in D \mid 1 \leq \indexproxy(x) \leq k\}$ as the $k$ nearest grs of the query object w.r.t. proxy distance. 

We define \textit{core set} as the set of all oracle neighbors whose proxy prefix is a valid answer. A core set $C$ is \textit{closed} w.r.t. an RT (resp. PT) query if for any $x \in C$, any oracle neighbor whose proxy index is larger (resp. smaller) than that of $x$ is also an element of $C$. {\sc Core Set Closure} assumes that, \textit{for any given query, the core set is closed}.

For RT queries, the core set is always closed, because as the proxy index of oracle neighbors increases, the recall of corresponding proxy prefix monotonically increases.
For PT queries, with a properly tuned proxy, the core set is likely to be closed in practice. We study the more general setting where core set may not be closed in \S~\ref{subsubsec:cse}. 


% We first give the definition for \textit{core set},
% \begin{definition}
% Given a query,
% \begin{enumerate}
%     \item A core set $C$ is the set of all oracle neighbors whose proxy prefix is a valid answer, i.e., $C=\{x \in \nearneighbor \mid \measure(\topproxy{\indexproxy(x)}) \geq \gamma\}$. 
%     \item A core set $C$ is \textit{upward closed} provided $\forall x_i \in C, \forall x_j \in \nearneighbor$, if $\indexproxy(x_i) \leq \indexproxy(x_j)$, then $x_j \in C$.
%     \item Symmetrically, a core set $C$ is \textit{downward closed} provided $\forall x_i \in C, \forall x_j \in \nearneighbor$, if $\indexproxy(x_j) \leq \indexproxy(x_i)$, then $x_j \in C$.
% \end{enumerate}
% \end{definition}

% We perform \textit{sample} and \textit{probe} to return answers (see \S~\ref{sec:approach}). Denote $\sunion$ as the union of all samples. 
Recall that $\kunion$ is the largest (resp. smallest) $\indexproxy(x)$ for RT (resp. PT) queries, where $x$ is an oracle neighbor in the union of all samples $\sunion$ (see \S~\ref{sec:approach}).
% $\kunion = \max \{\indexproxy(x) \mid x \in \sunion \land dist^O(x) \leq r\}$ for RT queries, and $\kunion = \min \{\indexproxy(x) \mid x \in \sunion \land dist^O(x) \leq r\}$ for PT queries , where $\sunion$ is the union of all samples.
% Given a uniformly drawn sample $S \subseteq D$, define $k_S = \max \{\indexproxy(x) \mid x \in S \land dist^O(x) \leq r\}$ for RT queries and $k_S = \min \{\indexproxy(x) \mid x \in S \land dist^O(x) \leq r\}$ for PT queries. 
If the core set $C$ is closed w.r.t. a given query, the success probability of $\topproxy{\kunion}$ equals to the likelihood of $\sunion$ intersecting with $C$, i.e., $\pos(\topproxy{\kunion}, \measure, \gamma) = Pr[\sunion \cap C \neq \varnothing]$. This can be easily examined by definition. Given a query, for core set $C$, we denote $|C|=c$.
Since samples are drawn uniformly, we have $Pr[\sunion \cap \closure \neq \varnothing] = 1 - (\binom{|D|-c}{s} / \binom{|D|}{s})^m = 1 - (\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})^{m}$, where $s$ is the sample size and $m$ is the number of samples. We denote $\poi(|D|,s,m,c) = 1 - (\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})^{m}$ for brevity.
% We have the following proposition,
% \begin{proposition} \label{prop:core_set}
% If the core set $C$ is upward closed for an RT query or downward closed for a PT query, $\pos(\topproxy{\kunion}, \measure, \gamma) = Pr[\sunion \cap C \neq \varnothing]$
% \end{proposition}

% Proposition \ref{prop:core_set} provides a way to compute the success probability of $\topproxy{\kunion}$. For RT queries, the core set is always upward closed, which comes from the monotonicity of recall measures. For PT queries, with a properly tuned proxy, the core set is likely to be downward closed. 
% Since we want to deliver high quality answers, we first study the situation when core set closure holds for both PT and RT queries. Formally, we have the assumption:
% \begin{assumption} [Core Set Closure]
% \label{assump:core_set_closure}
% Core sets are upward closed for RT queries, and downward closed for PT queries.
% \end{assumption}
% We further assume core sets are non-empty for simplicity. We study the general setting where core sets could be empty and Assumption \ref{assump:core_set_closure} may not hold in \S~\ref{subsubsec:cse}. 
% Under that assumption \ref{assump:core_set_closure}, we now present \csa, a unified approach to find high quality answers w.h.p. with a minimal oracle calls for RT and PT queries.

Next, we develop Algorithm \csa to find the optimal values $s=s^*$ and $m=m^*$, which ensures high success probability with a minimal expected oracle usage.


% A proposition for RT queries is as follows,
% \begin{proposition} [RT Upward Closure ] \label{prop:rt_up}
% Given an \query RT query, the largest core set is upward closed.
% \end{proposition}
% Proposition \ref{prop:rt_up}  We have the assumption,

% \begin{assumption} [PT Downward Closure] \label{asm:pt_down}
% Given an \query PT query, the largest core set is downward closed.
% \end{assumption}

% Assumption \ref{asm:pt_down} holds in situations when the proxy model is properly chosen and has high accuracy. Later in Section~\ref{subsubsec:cse}, we also study the situation in which Assumption \ref{asm:pt_down} may not hold and show how to ensure high success probability.

\subsubsection{\csa}
\label{subsubsec:csa}

% A useful schema to find answers to a given query is as follows. Given $1\leq s \leq |D|$, draw a sample $S \subseteq D$ of $|S|=s$ to estimate an index threshold $k_S$ and return $\topproxy{k_S}$ as the answer~. 
% We consider a general schema to find high quality answers to a query. 
% Given $1\leq s \leq |D|$ and a positive integer $m$, draw $m$ samples from $D$ at the size of $s$, denoted as, $S_1, S_2, \cdots, S_m$. Let $\sunion_{s,m}=\bigcup_{i=1}^{m} S_i$. We use $\sunion$ when $s$ and $m$ are clear for the context.
% We derive $\kunion$ from $\sunion$ and return $\topproxy{\kunion}$ as the answer. For RT queries, we denote $\kunion = \max \{\indexproxy(x) \mid x \in \sunion \land dist^O(x) \leq r\}$; for PT queries, let $\kunion = \min \{\indexproxy(x) \mid x \in \sunion \land dist^O(x) \leq r\}$. 
% We are interested in how to find the optimal pair of $s$ and $m$ to ensure high success probability with a minimal expected number of oracle calls.

% Given an \query query, for any $\topproxy{\kunion}$ derived from the aforementioned schema, we have
% \begin{small}
% \begin{equation}
% \label{eq:csa_prob}
% \begin{split}
% \pos(\topproxy{\kunion}, M, \gamma) = Pr[\sunion \cap \closure \neq \varnothing] &= 1 - (\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})^{m}\\
% \end{split}
% \end{equation}
% \end{small}
% where $C \subseteq D$ is the core set for the given query and $|C|=c$. We denote $\poi(|D|,s,m,c) = 1 - (\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})^{m}$ for brevity.

Given $s$ and $m$, the expected number of oracle calls is denoted as $\eou(s,m)=\mathbb{E}[|\sunion|]= |D|(1 - (1-\frac{s}{|D|})^{m})$. 
% We have
% \begin{small}
% \begin{equation}
% \begin{split} 
%     \eou(s,m)=\mathbb{E}[|\sunion|]
%     % & = \mathbb{E}[\sum_{x \in D} \mathbf{1}_{x \in \mathcal{S}_{s,m}}] = \sum_{x \in D} \mathbb{E}[\mathbf{1}_{x \in \mathcal{S}_{s,m}}]
%     = |D|(1 - (1-\frac{s}{|D|})^{m})\\
% \end{split}
% \end{equation}
% \end{small}
We want to find $s=s^*$ and $m=m^*$ which ensures $\poi(|D|,s,m,c) \geq 1 - \delta$ while
minimizing $\eou(s,m)$. Formally, we want to solve the problem,
\begin{small}
\begin{equation}
\label{problem:find_opt_s_m}
\begin{split} 
     \min_{s,m} \quad & \eou(s,m)=|D|(1 - (1-\frac{s}{|D|})^{m})\\
    \textrm{s.t.} \quad &\poi(|D|,s,m,c) \geq 1 - \delta   \\
\end{split}
\end{equation}
\end{small}

By plugging the expression of $\poi(|D|,s,m,c)$, the constraint can be simplified as $m \geq \lceil \frac{log(\delta)}{log(\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})} \rceil$, denoted as $m \geq \mlow(s)$ for brevity.
Note $\eou(s,m)$ monotonically increases as $m$ increases.
For a fixed $s$, the optimal $m$ which ensures a high success probability and minimizes $\eou(s,m)$ is taken by $m=\mlow(s)$. 
% \begin{small}
% \begin{equation}
%     m \geq \frac{log(\delta)}{log(\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})}
% \end{equation}
% \end{small}
% $\mlow(s)$ denotes the smallest $m$ value s.t. $\poi(|D|,s,m,c) \geq 1 - \delta$,
% \begin{small}
% \begin{equation}
%     \mlow(s) = \lceil \frac{log(\delta)}{log(\prod_{i=0}^{c-1} \frac{|D|-s-i}{|D|-i})} \rceil
% \end{equation}
% \end{small}
Importantly, we have $m^*=\mlow(s^*)$.
In light of this, we can solve Problem \ref{problem:find_opt_s_m} procedurally by comparing $\eou(s,m)$ for each $1\leq s \leq |D|$ and $m=\mlow(s)$. 

Such exhaustive search for the exact value of $s^*$ and $m^*$, however, can be expensive in large DB. Instead, we are interested in approximation solutions with good guarantees. 
% In order to ensure high success probability, we have $s \geq \frac{-log(\delta)}{\sum_{i=0}^{c-1} \frac{m}{|D|-i}}$. Since $\eou(s,m)$ monotonically increases as $s$ increases, similarly, we denote $\slow(m) = \lceil \frac{-log(\delta)}{\sum_{i=0}^{c-1} \frac{m}{|D|-i}} \rceil$ as a lower bound for $s$ to ensure high success probability for a given $m$.
Given a query, 
we define $\xi = \frac{|D|-\eou(s,m)}{|D|-\eou(s^*, m^*)}$ as the approximation ratio for any $s$ and $m$, which accounts for saved oracle usage in comparison to calling oracle on the whole DB.
A larger $\xi$ indicates a better approximation solution, and the optimum $s=s^*$ and $m=m^*$ gives $\xi = 1$.


Typically, we are interested in the case either $s=1$ or $m=1$. 
For $s=1$, we choose $m=\mlow(1)$, and 
\begin{small}
\begin{equation}
     \xi_{s=1} \geq \delta^{\frac{-1}{c}( \frac{1}{|D|} - \frac{|D|}{|D|-1})} \cdot (1-\frac{1}{|D|})
\end{equation}
\end{small}
For $m=1$, we choose $s=\lceil \frac{-log(\delta)}{\sum_{i=0}^{c-1} \frac{1}{|D|-i}} \rceil$ to ensure high success probability, and 
% Similarly, for a fixed $m$, the smallest $s$ ensuring a high success probability has $s \geq \frac{-log(\delta)}{\sum_{i=0}^{c-1} \frac{m}{|D|-i}}$. We denote $\slow(m) = \lceil \frac{-log(\delta)}{\sum_{i=0}^{c-1} \frac{m}{|D|-i}} \rceil$ for any given $m$.
% For $m=1$, we use $s=\slow(1)$, then
\begin{small}
\begin{equation}
\label{eq:csa_m1}
    \xi_{m=1} \geq  \delta ^{\frac{-1}{|D|c}} \cdot (1 - \frac{1}{|D|} + \frac{log(\delta)}{c})
\end{equation}
\end{small}

In a practical setting where $\delta=0.1$, $|D|=10000$, and $c=100$, we have both $\xi_{s=1}$ and $\xi_{m=1}$ being no less than $97.7\%$, that is, if we fix either $s=1$ or $m=1$ as above, the saved oracle usage is at least $97.7\%$ of that $s^*$ and $m^*$ can achieve. 
We perform a detailed study on these two settings with real-world datasets in \S~\ref{subsec:csa}.

\csa is presented in Algorithm \ref{alg:csa}. We compute $s^*$ and $m^*$ in line \ref{csa:getsm} either exactly or approximately as demanded, and draw samples accordingly in line \ref{csa:sample}. In lines \ref{csa:comp_k} to \ref{csa:e}, we compute $\kunion$ according to the query type and return $\topproxy{\kunion}$ as the answer.
\normalem
\begin{algorithm}
\caption{\csa}
\label{alg:csa}

\DontPrintSemicolon
  \SetKwFunction{fcsa}{CSC}
  \SetKwProg{Fn}{Function}{:}{}
  \SetKwFunction{sample}{UniformSample}
  \SetKwFunction{fsm}{getsm}
  
\Fn{\fcsa{$D$, $c$, $\delta$}}{
$s^*, m^* \gets$ \fsm{$|D|$, $c$, $\delta$}\; \label{csa:getsm}
$\sunion \gets$ \sample{$D$, $s^*$, $m^*$}\; \label{csa:sample}
\eIf{RT query \label{csa:comp_k}}
{$\kunion \gets \max \{ I(x) \mid x \in \sunion \land dist^O(x) \leq r  \}$}
{$\kunion \gets \min \{ I(x) \mid x \in \sunion \land dist^O(x) \leq r  \}$}
\KwRet $\topproxy{\kunion}$
\label{csa:e}}
\end{algorithm}
\ULforem

\subsubsection{\cse}
\label{subsubsec:cse}
Given a query, \cse extends \csa to find high probability valid answers in general settings.
% calibrates the core set size $c$ and invokes \csa to find high probability valid answers. 

For RT queries, since core sets are always closed, \cse-RT estimates core set sizes and invokes \csa to find valid answers w.h.p.
% we can derive a confidence interval for the core set size. For core set $C$, denote $|C|=c$. 
% Recall core set comprises all oracle neighbors of proxy prefix being a valid answer.
For an RT query with target $\gamma$, the core set $C$ consists of the top $(1-\gamma)\times 100$ \% oracle neighbors of largest proxy indices. That is, $c=\lfloor |\nearneighbor|(1-\gamma)\rfloor+1$. 
We show how to estimate a likely lower bound for $c$ by drawing samples and applying Hoeffding Bounds \cite{vershynin_2018}.
\begin{proposition} [Hoeffding Bounds] 
Let $\{X_i\}_{i=1}^{n}$ be independent random variables and that, $X_i \in \{0,1\}$ and $\mathbb{E}[X_i] = \mu$.Let $\hat{\mu} = \frac{1}{n} \sum_{i=1}^n X_i$. For $\forall \epsilon \geq 0$, we have the concentration bound
\begin{small}
\begin{equation}
    Pr[\hat{\mu}-\epsilon \leq \mu] \geq 1-exp(-2n\epsilon^2)
\end{equation}
\end{small}
\end{proposition}

% Let $\mud = \frac{|\nearneighbor|}{|D|}$.
Randomly draw $x_i \in D$. Let $X_i = 1$ iff $dist^O(x_i) \leq r$. We have $\mathbb{E}[X_i] = \frac{|\nearneighbor|}{|D|}$, denoted as $\mud$. We randomly draw $\{x_i\}_{i=1}^{n}$ with replacement and denote $\hat{\mud} = \frac{1}{n} \sum_{i=1}^n X_i$. 
For any $\epsr, \deltar \in (0,1)$, by Hoeffding Bounds, we have $Pr[\hat{\mud}-\epsr \leq \mud] \geq 1-\deltar $ if $n \geq \frac{log(\deltar)}{-2\epsr^2}$. Equally, we have $Pr[c\geq \lfloor |D|(\hat{\mud}-\epsr)(1-\gamma)\rfloor+1]\geq 1-\deltar$, if $n \geq \frac{log(\deltar)}{-2\epsr^2}$. We denote the lower bound $\clow := \lfloor |D|(\hat{\mud}-\epsr)(1-\gamma)\rfloor+1$.

Next, we call \csa to return answers by solving a similar minimization problem w.r.t. $\clow$ and $\frac{1-\delta}{1-\deltar}$,
\begin{small}
\begin{equation}
\label{prb:csert}
\begin{split} 
     \min_{s,m} \quad & \eou(s,m)=|D|(1 - (1-\frac{s}{|D|})^{m})\\
    \textrm{s.t.} \quad &\poi(|D|,s,m,\clow) \geq \frac{1-\delta}{1-\deltar}  \\
\end{split}
\end{equation}
\end{small}
% Let $s^*$ and $m^*$ be the optimal solution to Problem \ref{prb:csert}, and $\sunion^*$ is the corresponding union of samples. 
The returned answer satisfies validity for any given query with a probability no less than $1 - \delta$.
% \begin{small}
% \begin{equation} 
% \begin{split}
% \pos(\topproxy{\kunion[\sunion^*]}, \recall, \gamma) 
% &= Pr[\sunion^* \cap \closure \neq \varnothing] 
%     % &\geq Pr[\sunion^* \cap \closure \neq \varnothing \land c \geq \clow ] \\
%     % &=Pr[\sunion^* \cap \closure \neq \varnothing \mid c \geq \clow ] \cdot Pr[c \geq \clow] \\
%     \geq \poi(|D|,s^*,m^*,\clow) \cdot (1-\deltar)
%     % &\geq \frac{1-\delta}{1-\deltar} \cdot (1-\deltar)\\
%     % = 1-\delta
% \end{split}
% \end{equation}
% \end{small}
% Since $\poi(|D|,s^*,m^*,\clow) \geq \frac{1-\delta}{1-\deltar}$, we have $\pos(\topproxy{\kunion[\sunion^*]}, M, \gamma) \geq 1-\delta$.

For PT queries, core sets may not be closed in general and we cannot ensure high success probability by simply calling \csa. 
Instead, we use \csa as a good heuristic to find answer candidates, and apply Hoeffding Bounds to ensure the returned answer is valid w.h.p. 
Specifically, given a query, we estimate $c$ by sampling and probing, and compute an answer candidate $\topkproxy{k_1}$ by calling \csa. 
We also use the same sample to estimate the largest $k$ where $\topkproxy{k}$ meets sampled validity, denoted as $k_2$.
To improve CR (i.e., recall), we denote $\hat{k}=\max\{k_1, k_2\}$ and consider $\topkproxy{\hat{k}}$.
Next, we draw samples and estimate a likely lower bound of $\precis(\topkproxy{\hat{k}})$ by applying Hoeffding Bounds.
For a PT query with target $\gamma$, we return $\topproxy{\hat{k}}$ if the estimated lower bound is no less than $\gamma$ w.h.p. Otherwise, we return all oracle neighbors identified from samples.

\normalem
\begin{algorithm}
\caption{CSE}
\label{alg:cse}
\DontPrintSemicolon
  \SetKwFunction{fcsert}{CSE-RT}
\SetKwFunction{fcsept}{CSE-PT}
  \SetKwProg{Fn}{Function}{:}{}
  \SetKwFunction{sample}{UniformSample}
%   \SetKwFunction{fcsa}{CSC}
  \SetKwFunction{fhb}{HoeffdingEst}

\Fn{\fcsert{$D$, $\delta$} \label{csert:s}}
{
$\hat{\mud} \gets$ \fhb{$D$, $\deltar$, $\epsilon_r$} \;
$\clow \gets \lfloor |D|(\hat{\mud}-\epsilon_r)(1-\gamma)\rfloor+1$\;

\KwRet \fcsa{$D$, $\clow$, $\frac{1-\delta}{1-\deltar}$}
\label{csert:e}}
  
\Fn{\fcsept{$D$, $\delta$}\label{csept:s}}
{
$S \gets$ \sample{$D$, $b=100$}\; \label{csept:sample}
$\hat{c} \gets \frac{|D|}{|S|} \cdot \text{the size of core set w.r.t. } S$\;
% \max\{ |S'| \mid S' \subseteq S \land S' \text{ is a lower core set} \} 
$\topproxy{k_1} \gets$ \fcsa{$D$, $\hat{c}$, $1-\delta$}\;\label{csept:est_topk}
$k_2 \gets \max\{ I(x) \mid x \in S \land M_p(\topkproxy{I(x)} \cap S) \geq \gamma \}$\; \label{csept:khat}
$\hat{k} \gets \max\{ k_1, k_2\}$\;\label{csept:kstar}
$\underline{\mu_{\topproxy{\hat{k}}}} \gets$ \fhb{$\topproxy{\hat{k}}$, $\delta$, $\epsilon_p$} $- \epsilon_p$ \label{csept:hb}

\eIf{$\underline{\mu_{\topproxy{\hat{k}}}} \geq \gamma$}
{\KwRet $\topproxy{\hat{k}}$}
{\KwRet $\{x \in S \mid dist^O(x) \leq r\}$}
\label{csept:e}}

\Fn{\fhb{$D$, $\delta$, $\epsilon$}}{
$S \gets$ \sample{$D$, $\lceil \frac{log(\delta)}{-2\epsilon^2} \rceil$}\;
\KwRet $\hat{\mu} \gets \frac{|\{x \in S \mid dist^O(x) \leq r\}|}{|S|}$\;
}

\end{algorithm}
\ULforem

The algorithm of \cse is given in Algorithm \ref{alg:cse}.
\cse-RT is given in lines \ref{csert:s} to \ref{csert:e}. We first estimate $\hat{\mud}$ by drawing samples and applying Hoeffding Bounds, and then compute $\clow$ and return answers by calling \csa. 
\cse-PT is given in line \ref{csept:s} to \ref{csept:e}. In line \ref{csept:sample} to \ref{csept:est_topk}, we draw samples to derive the estimation $\hat{c}$ and compute $\topproxy{k_1}$ by calling \csa. In lines \ref{csept:khat} to \ref{csept:kstar}, we use the same sample to estimate $k_2$ and choose $\hat{k}$ as the maximum of $k_1$ and $k_2$. In lines \ref{csept:hb} to \ref{csept:e}, we derive a likely lower bound for the precision of $\topkproxy{\hat{k}}$ by drawing samples and applying Hoeffding Bounds. We return $\topproxy{\hat{k}}$ if the lower bound is no less than the target $\gamma$. Otherwise, we return all oracle neighbors of the query object identified from samples.

By design, \csa finds high probability valid answers with a minimal expected oracle usage, when core sets are closed w.r.t. the given query. \cse extends \csa to situations where core sets may not be closed, and finds high probability valid answers by applying Hoeffding Bounds. 

\eat{
\section{Algorithms}
\label{sec:algos}
We provide the details of our theoretical analysis and algorithms. 

\subsection{Algorithms with Proxy Quality Assumption}
\label{subsec:algos-assumption}

We first present our assumption on proxy model quality, under which we show how to compute the optimal valid answer set which maximizes the expected CR with no oracle cost. We propose algorithms for both PT and RT queries, whose complexity are $O(|D|^3)$.

The assumption we will use is as follows. Consider a dataset $D = \{p_1, p_2, \cdots, p_{|D|}\}$ and a given query object $q$, we assume,

\begin{assumption} [Proxy Quality Assumption]
\label{proxy_quality_assumption}
\begin{equation}
dist(O(q), O(p_i)) = dist(O(q), T(p_i)) + \epsilon_i, \,  i=1,2,\cdots, |D|
\end{equation}
where $\epsilon_i$ are i.i.d., $\epsilon_i \sim \mathcal{X}$. 
\end{assumption}
For simplicity of language, we use \textit{proxy distance} to denote $dist(O(q), T(p_i))$ and \textit{oracle distance} to denote $dist(O(q), O(p_i))$ whenever the context is clear.
Assumption \ref{proxy_quality_assumption} assumes, for any $p_i \in D$, the difference between its oracle distance and proxy distance are i.i.d. random variables drawn from a known distribution $\mathcal{X}$. Let $\Phi(x)$ be the cdf of distribution $\mathcal{X}$.

The problem we are going to solve is as follows,
\begin{problem} [PT/RT-query With Quality Assumption]
\label{problem:ptrt_w_assump}
Given a PT/RT-query $Q$, if Assumption \ref{proxy_quality_assumption} holds, find the \textbf{valid} answer which \textbf{maximizes $\mathbb{E}[CR]$} with \textbf{zero oracle invocation}.
\end{problem}

We define an indicator function $\mathbf{1}(p_i)=1$ iff $dist(O(q), O(p_i)) \leq t$ for a given $t$ and $p_i \in D$. Under Assumption \ref{proxy_quality_assumption}, we have the following facts,
\begin{fact}
\label{fact:identity}
\begin{equation}
\begin{split}
Pr[\mathbf{1}(p_i)=1]&=Pr[dist(O(q), O(p_i)) \leq t]\\
&=Pr[dist(O(q), T(p_i)) + \epsilon_i \leq t]\\
&=Pr[\epsilon_i \leq t-dist(O(q), T(p_i))]\\
&=\Phi(t-dist(O(q), T(p_i))), \, i=1,2,\cdots, |D|
\end{split}
\end{equation}
\end{fact}

\begin{fact}
\label{fact:precision_recall}
For any real number $\gamma \in (0,1)$ and subset $S \subseteq D$ of size $s$,
\begin{equation}
\label{eq:precis_prob}
\begin{split}
    Pr[Precision(S) \geq \gamma] &= Pr[\frac{\sum_{p_i \in S} \mathbf{1}(p_i)}{|S|} \geq \gamma]\\
    &=Pr[\sum_{p_i \in S} \mathbf{1}(p_i) \geq \lceil s\gamma \rceil] \\
\end{split}
\end{equation}
\begin{equation}
\label{eq:recall_prob}
\begin{split}
    Pr[Recall(S) \geq \gamma] &= 
    \sum_{j=0}^{s} Pr[\sum_{p_i \in S} \mathbf{1}(p_i)=j]\cdot Pr[\sum_{p_i \in D \setminus S} \mathbf{1}(p_i) \leq \lfloor \frac{(1-\gamma)j}{\gamma} \rfloor]\\
\end{split}
\end{equation}
\end{fact}

Fact \ref{fact:identity} gives the likelihood for a given object $p_i$ having small oracle distance. We use $\phi(p_i) := \Phi(t-dist(O(q), T(p_i)))$ to denote this likelihood, or $\phi_i$ whenever the context is clear.
Fact \ref{fact:precision_recall} presents how to compute the success probability for both query types w.r.t. a specific subset $S$ and target rate $\gamma$. 
The computation of $Pr[Precision(S) \geq \gamma]$ and $Pr[Recall(S) \geq \gamma]$ involves the probability distribution of the summation $\sum_{p_i \in S} \mathbf{1}(p_i)$ for a given $S\subseteq D$, which turns out to be a poisson binomial random variable \cite{fernandez2010poisson}.

Given that, our algorithm first computes the probability distribution for $\sum_{p_i \in S} \mathbf{1}(p_i)$, with which we can derive $Pr[Precision(S) \geq \gamma]$ and $Pr[Recall(S) \geq \gamma]$ in $O(s)$ and $O(s|D|)$ separately for any given $S$ and $\gamma$. We use \textit{direct convolution} method proposed in \cite{osti_1548776} to compute the probability distribution. 

Suppose we have $S = \{p_1, p_2, \cdots, p_s\}$ and $p_{s+1} \in D \setminus S$. For $0 \leq k \leq s+1$, the following relation holds,
\begin{equation}
\label{eq:pndist_update}
\begin{split}
    Pr[\sum_{p_i \in S \cup \{p_{s+1}\}} \mathbf{1}(p_i) = k] = &Pr[\sum_{p_i \in S} \mathbf{1}(p_i) = k-1]\cdot \phi_{s+1} + \\
    &Pr[\sum_{p_i \in S} \mathbf{1}(p_i) = k]\cdot (1-\phi_{s+1})\\
\end{split}
\end{equation}
which can be used to compute the distribution of $\sum_{p_i \in S \cup \{p_{s+1}\}} \mathbf{1}(p_i)$ from $\sum_{p_i \in S} \mathbf{1}(p_i)$ in $O(s)$ time. We start from $S'=\{p_1\}$ where the distribution is $Pr[\sum_{p_i \in S'} \mathbf{1}(p_i) = 0] = 1-\phi_1$ and $Pr[\sum_{p_i \in S'} \mathbf{1}(p_i) = 1] = \phi_1$. Next, we continue adding elements $p_2, p_3, \cdots, p_s$ into $S'$ and update the distribution through equation \ref{eq:pndist_update}. It is clear that we need to compute $s$ distributions and the overall time complexity is $O(s^2)$. More details can be found in Algorithm \ref{alg:compute_pndist}.

\begin{algorithm}
\caption{Compute Possion Binomial Distribution }
\label{alg:compute_pndist}
% \begin{algorithmic} [1]
% \Procedure{PBDistribution}{$S = \{p_1, p_2, \cdots, p_s\}$}
% \State $PB \gets \Call{Zeros}{size=s+1}$
% \State $PB[0] \gets 1-\phi_1$; $PB[1] \gets \phi_1$
% \label{pbdist:init}
% \For{$i \gets 2, 3, \cdots, s$}
% \label{pbdist:convl_s}
%     \For{$j \gets 0, 1, \cdots, i$}
%         \State $PB[j] \gets PB[j](1-\phi_{i}) + PB[j-1]\phi_i$
%     \EndFor
% \EndFor
% \label{pbdist:convl_e}
% \State \Return $PB$
% \EndProcedure
% \end{algorithmic}
\end{algorithm}
In line \ref{pbdist:init}, we initializes the probability distribution vector $PB$ with the probability distribution of $\mathbf{1}(p_1)$. In line \ref{pbdist:convl_s} to \ref{pbdist:convl_e}, we iteratively include $p_2, p_3, \cdots, p_s$ and update $PB$ accordingly.

After obtaining the probability distribution for $\sum_{p_i \in S} \mathbf{1}(p_i)$, we can compute the cdf $Pr[\sum_{p_i \in S} \mathbf{1}(p_i) \leq k]$ or the survival function $Pr[\sum_{p_i \in S} \mathbf{1}(p_i) \geq k]$ for any given $0 \leq k \leq s$ by summing over the probability distribution vector in $O(s)$ time. In light of this, we can compute $Pr[Precision(S) \geq \gamma]$ and $Pr[Recall(S) \geq \gamma]$ by utilizing the Fact \ref{fact:precision_recall}. The algorithms are given as Algorithm \ref{alg:compute_precision} and Algorithm \ref{alg:compute_recall}.

\begin{algorithm}
\caption{Compute $Pr[Precision(S) \geq \gamma]$}
\label{alg:compute_precision}
% \begin{algorithmic} [1]
% \Procedure{PBPrecision}{$S = \{p_1, p_2, \cdots, p_s\}, \gamma$}
% \State $PB \gets \Call{PBDistribution}{S}$
% \State $prob\_precis \gets \Call{Sum}{PB[\lceil s\gamma \rceil], PB[\lceil s\gamma \rceil + 1], \cdots, PB[s]}$
% \State \Return $prob\_precis$
% \EndProcedure
% \end{algorithmic}
\end{algorithm}

\begin{algorithm}
\caption{Compute $Pr[Recall(S) \geq \gamma]$}
\label{alg:compute_recall}
% \begin{algorithmic} [1]
% \Procedure{PBRecall}{$S = \{p_1, p_2, \cdots, p_s\}, D, \gamma$}
% \State $PB_S \gets \Call{PBDistribution}{S}$
% \State $PB_{SC} \gets \Call{PBDistribution}{D \setminus S}$
% \State $prob\_recall \gets 0$
% \For{$j \gets 0, 1, 2, \cdots, s$}
%     \State $CDF_{SC} \gets \Call{Sum}{PB_{SC}[0], PB_{SC}[1], \cdots, PB_{SC}[\lfloor \frac{(1-\gamma)j}{\gamma} \rfloor]}$
%     \State $prob\_recall \gets prob\_recall + PB_S[j] \cdot CDF_{SC} $
% \EndFor
% \State \Return $prob\_recall$
% \EndProcedure
% \end{algorithmic}
\end{algorithm}

The implementation of Algorithm \ref{alg:compute_precision} and \ref{alg:compute_recall} is a direct application of Fact \ref{fact:precision_recall}.
It can be easily examined that Algorithm \ref{alg:compute_precision} is dominated by the computation of $PB$, which is of $O(s^2)$ time complexity; Algorithm \ref{alg:compute_recall} is dominated by the computation of $PB_{S}$ and $PB_{SC}$, which is of $O(|D|^2)$ time complexity.

Now we have seen how to compute $Pr[Precision(S) \geq \gamma]$ and $Pr[Recall(S) \geq \gamma]$ for a given subset $S\subseteq D$. Next, we are going to solve the problem \textit{how to find $S \subseteq D$ which maximizes $\mathbb{E}[CR]$ while $Pr[Precision(S) \geq pt] \geq prob$ for PT-query, or $Pr[Recall(S) \geq rt] \geq prob$ for RT-query, respectively}.

Note that a naive algorithm to this problem is enumerating all possible $S \subseteq D$ and computing both success probability and expectation to return the optimal answer,
which takes at least $2^{|D|}$ operations. Such exponential algorithm is prohibitively expensive even for moderate dataset size. We propose a $O(|D|^3)$ algorithm for both PT-query and RT-query by showing several monotonic properties of success probability and expected CR for a given answer set. At first, we want to prove the following lemma,

\begin{lemma} [Monotonicity of Replacement]
\label{lemma:monoto_replace}
Given a subset $S \subseteq D$ and $\gamma \in (0,1)$, for $p_j \in S$ and $p_k \in D \setminus S$, if $\phi_j \leq \phi_k$, then
\begin{equation}
\begin{split}
     Pr[Precision(S) \geq \gamma] &\leq Pr[Precision(S \cup \{p_k\} \setminus \{p_j\}) \geq \gamma]\\
     Pr[Recall(S) \geq \gamma] &\leq Pr[Recall(S \cup \{p_k\} \setminus \{p_j\}) \geq \gamma]\\
\end{split}
\end{equation}
\end{lemma}

The intuition is simple, if we replace a ``bad'' object with a likely ``better'' object in the answer set, both precision and recall rates are likely to get improved. In order to prove Lemma \ref{lemma:monoto_replace}, we need to introduce the notion of the \textit{usual stochastic order} 
, $\leq_{st}$.

\begin{definition} [Usual Stochastic Order]
\label{def:usual_stocha_order}
Let $X$ and $Y$ be two random variables such that,
\begin{equation}
    Pr[X \geq x] \leq Pr[Y \geq x], \, \forall x\in (-\infty, \infty).
\end{equation}
Then $X$ is said to be smaller than $Y$ in the usual stochastic order (denoted by $X \leq_{st} Y$).
\end{definition}

One important property for usual stochastic order is as follows,

\begin{proposition} 
\label{prop:st_expectation}
Let $X$ and $Y$ be two random variables. If $X \leq_{st} Y$, then 
\begin{equation}
    \mathbb{E}[\psi(X)] \leq \mathbb{E}[\psi(Y)]
\end{equation}
for all \textit{increasing function} $\psi$ for which the expectations exist.
\end{proposition}

The proof of Proposition \ref{prop:st_expectation} relies on constructing upper sets on the domain of $X$ and $Y$, which is beyond the scope of this paper. We refer interested readers to the literature  for more details.

Now, we can prove Lemma \ref{lemma:monoto_replace}.
\begin{proof}
Denote $S' = S \cup \{p_k\} \setminus \{p_j\}$.
We are going to prove a stronger result, that is $Precision(S) \leq_{st} Precision(S')$ and $Recall(S) \leq_{st} Recall(S')$.

% Consider the case $\gamma \in (-\infty, 0]$. We have $Pr[Precision(S') \geq \gamma] = Pr[Precision(S) \geq \gamma] = 1$, and $Pr[Recall(S') \geq \gamma] = Pr[Recall(S) \geq \gamma] = 1$. Thus,
% \begin{equation}
% \begin{split}
%      Pr[Precision(S) \geq \gamma] &\leq Pr[Precision(S') \geq \gamma]\\
%      Pr[Recall(S) \geq \gamma] &\leq Pr[Recall(S') \geq \gamma]\\
% \end{split}
% \end{equation}

% Similarly, when $\gamma \in (1, \infty)$, all probabilities above take the value of $0$ and we have the same inequality hold. The last piece of puzzle is when $\gamma \in (0, 1]$. 
We are going to first discuss precision, and then the recall.

For precision, define random variables $X=\sum_{p_i \in S \setminus \{p_j\}} \mathbf{1}(p_i)$, $Y=X+\mathbf{1}(p_j)$, and $Z=X+\mathbf{1}(p_k)$. By plugging equation \ref{eq:precis_prob}, we can rewrite $Pr[Precision(S)\geq \gamma]$ as $Pr[Y \geq \lceil s\gamma \rceil]$ and
\begin{equation}
\label{eq:prob_expand_trick}
\begin{split}
Pr[Y \geq \lceil s\gamma \rceil]
    &= Pr[X \geq \lceil s\gamma \rceil \land \mathbf{1}(p_j)=0] + Pr[X \geq \lceil s\gamma \rceil-1 \land \mathbf{1}(p_j)=1] \\
    &= Pr[X \geq \lceil s\gamma \rceil](1-\phi_j) + Pr[X \geq \lceil s\gamma \rceil-1]\phi_j\\
    &= \phi_j \cdot Pr[X=\lceil s\gamma \rceil-1] + Pr[X \geq \lceil s\gamma \rceil]
\end{split}
\end{equation}
where the last step is due to $Pr[X \geq \lceil s\gamma \rceil-1] - Pr[X \geq \lceil s\gamma \rceil] = Pr[X=\lceil s\gamma \rceil-1]$. Following a similar procedure, we can rewrite $Pr[Precision(S')\geq \gamma]$ as $Pr[Z \geq \lceil s\gamma \rceil]$ and 
\begin{equation}
    Pr[Z \geq \lceil s\gamma \rceil] = \phi_k \cdot Pr[X=\lceil s\gamma \rceil-1] + Pr[X \geq \lceil s\gamma \rceil]
\end{equation}

Since $\phi_j \leq \phi_k$, we have $Pr[Y \geq \lceil s\gamma \rceil] \leq Pr[Z \geq \lceil s\gamma \rceil]$ for $\gamma \in \mathbb{R}$, and therefore $Pr[Precision(S)\geq \gamma] \leq Pr[Precision(S')\geq \gamma]$ for $\gamma \in \mathbb{R}$. By definition \ref{def:usual_stocha_order}, we can conclude
\begin{equation}
    Precision(S) \leq_{st} Precision(S')
\end{equation}
and also $Y \leq_{st} Z$, which will help us to finish the proof for recall rates.

Next, we want to prove $Pr[Recall(S)\geq \gamma] \leq Pr[Recall(S')\geq \gamma]$ for $\gamma \in \mathbb{R}$. 

When $\gamma = 0$, we have $Pr[Recall(S)\geq 0] = 1 \leq Pr[Recall(S')\geq 0] = 1$.

When $\gamma \in \mathbb{R} \setminus \{0\}$, by denoting new random variables $X_C=\sum_{p_i \in D \setminus S \cup \{p_j\}} \mathbf{1}(p_i)$, $Y_C=X_C-\mathbf{1}(p_j)$, and $Z_C=X_C-\mathbf{1}(p_k)$, we can rewrite equation \ref{eq:recall_prob} as,
\begin{equation}
\begin{split}
    Pr[Recall(S) \geq \gamma] &= 
    \sum_{j=0}^{s} Pr[Y=j]\cdot Pr[Y_C \leq \lfloor \frac{j}{\gamma} \rfloor],\\
    Pr[Recall(S') \geq \gamma] &= 
    \sum_{j=0}^{s} Pr[Z=j]\cdot Pr[Z_C \leq \lfloor \frac{j}{\gamma} \rfloor].\\
\end{split}
\end{equation}
We are going to first prove $Pr[Z_C \leq \lfloor \frac{j}{\gamma} \rfloor]  \geq Pr[Y_C \leq \lfloor \frac{j}{\gamma} \rfloor]$ for any $0 \leq j \leq s$. We use the same trick as in equation \ref{eq:prob_expand_trick},
\begin{equation}
\begin{split}
Pr[Y_C \leq \lfloor \frac{j}{\gamma} \rfloor]
    &= Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor \land \mathbf{1}(p_j)=0] + Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor+1 \land \mathbf{1}(p_j)=1] \\
    &= Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor](1-\phi_j) + Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor+1]\phi_j\\
    &= \phi_j \cdot Pr[X_C = \lfloor \frac{j}{\gamma} \rfloor+1] + Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor]
\end{split}
\end{equation}
and 
\begin{equation}
\begin{split}
Pr[Z_C \leq \lfloor \frac{j}{\gamma} \rfloor]
    &= \phi_k \cdot Pr[X_C = \lfloor \frac{j}{\gamma} \rfloor+1] + Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor]
\end{split}
\end{equation}

Since $\phi_j \leq \phi_k$, we conclude $Pr[Y_C \leq \lfloor \frac{j}{\gamma} \rfloor]  \leq Pr[Z_C \leq \lfloor \frac{j}{\gamma} \rfloor]$ for any $0 \leq j \leq s$. 
By defining $\psi(x) := Pr[Z_C \leq \lfloor \frac{x}{\gamma} \rfloor]$, we can write the following inequality,
\begin{equation}
    Pr[Recall(S) \geq \gamma] \leq 
    \sum_{j=0}^{s} Pr[Y=j]\cdot \psi(j) =\mathbb{E}[\psi(Y)] .
\end{equation}
Because $Pr[Z_C \leq \lfloor \frac{x}{\gamma} \rfloor] = Pr[\gamma \cdot Z_C \leq x]$, which is the cdf for the random variable $\gamma Z_C$, we know $\psi(x)$ is an increasing function. By applying Proposition \ref{prop:st_expectation} in addition to the result $Y \leq_{st} Z$ which we have proven above, we have,
\begin{equation}
    Pr[Recall(S) \geq \gamma] \leq \mathbb{E}[\psi(Y)] \leq \mathbb{E}[\psi(Z)] = Pr[Recall(S') \geq \gamma]
\end{equation}
for $\gamma \in \mathbb{R} \setminus \{0\}$. 

At last, we can conclude $Pr[Recall(S) \geq \gamma] \leq Pr[Recall(S') \geq \gamma]$ for $\gamma \in \mathbb{R}$ and therefore
\begin{equation}
    Recall(S) \leq_{st} Recall(S')
\end{equation}
\end{proof}

Lemma \ref{lemma:monoto_replace} characterizes the monotonicity of success probability when we replace ``bad'' objects with likely ``better'' objects. Since our problem also asks for a maximal expected CR, a natural question to ask is \textit{does there exist monotonicity of  $\mathbb{E}[CR]$ over replacement operation?} It turns out that we can prove the following lemma,

\begin{lemma} [Monotonicity of Expectation (Replacement)]
\label{lemma:monoto_expect_replace}
Given a subset $S \subseteq D$ and $\gamma \in (0,1)$, for $p_j \in S$ and $p_k \in D \setminus S$, if $\phi_j \leq \phi_k$, then
\begin{equation}
\begin{split}
\mathbb{E}[Precision(S)] &\leq \mathbb{E}[Precision(S \cup \{p_k\} \setminus \{p_j\})]\\
\mathbb{E}[Recall(S)] &\leq \mathbb{E}[Recall(S \cup \{p_k\} \setminus \{p_j\})]\\
\end{split}
\end{equation}
\end{lemma}

\begin{proof}
Let $S' = S \cup \{p_k\} \setminus \{p_j\}$. Since we have proven $Precision(S) \leq_{st} Precision(S')$ and $Recall(S) \leq_{st} Recall(S')$, by Proposition \ref{prop:st_expectation}, we have
\begin{equation}
\begin{split}
    \mathbb{E}[\psi(Precision(S))] &\leq \mathbb{E}[\psi(Precision(S'))] \\
    \mathbb{E}[\psi(Recall(S))] &\leq \mathbb{E}[\psi(Recall(S'))] \\    
\end{split}
\end{equation}
where $\psi(x)$ is an increasing function.

Let $\psi(x) := x$, we can conclude 
\begin{equation}
\begin{split}
    \mathbb{E}[Precision(S)] &\leq \mathbb{E}[Precision(S')] \\
    \mathbb{E}[Recall(S)] &\leq \mathbb{E}[Recall(S')] \\    
\end{split}
\end{equation}
\end{proof}

Lemma \ref{lemma:monoto_replace} and Lemma \ref{lemma:monoto_expect_replace} together hint at that, if we replace ``bad'' objects with likely ``better'' objects from an answer set, we can monotonically increase the success probability and expected CR values, which means a better solution. Recall that $\topkproxy{k} := \{ \text{top-k objects of smallest proxy distance} \}$, we can have the following lemma,

\begin{lemma} 
\label{lemma:topk}
For a given PT/RT-query, if $S\subseteq D$ of size $s$ is a valid answer, then $\topkproxy{s}$ is a valid answer and $\mathbb{E}[CR(\topkproxy{s})] \geq \mathbb{E}[CR(S)]$.
\end{lemma}

\begin{proof}
The proofs for PT and RT query are quite similar. We will prove the theorem for PT-query only and leave RT-query to readers.

Because $S \subseteq D$ is a valid answer, we have $Pr[Precision(S) \geq pt] \geq prob$. We want to prove that $D_s$ can be constructed from $S$ through a series of replacement operation, in each step we monotonically increase success probability and the expected CR. We use $S[k]$ to denote \textit{the object of the k-th smallest proxy distance in $S$}, and similar for $D_s[k]$.

An example series of replacement is as follows. Denote $S_0 := S$, we construct $S_i = S_{i-1} \setminus \{S[i]\} \cup \{D_s[i]\}$ for $i=1,2,\cdots,s$. By the definition of $D_s$, we know the proxy distance of $D_s[i]$ is smaller than $S[i]$. Because $\phi(p_i) = \Phi(t-dist(O(q), T(p_i)))$ for $p_i \in D$, which decreases when the proxy distance goes up, we have $\phi(D_s[i]) \geq \phi(S[i])$. According to Lemma \ref{lemma:monoto_replace} and \ref{lemma:monoto_expect_replace}, we have $Pr[Precision(S_i) \geq pt] \geq Pr[Precision(S_{i-1}) \geq pt]$ and $\mathbb{E}[CR(S_i)] \geq \mathbb{E}[CR(S_{i-1})]$ for $i=1,2,\cdots, s$. Note $D_s = S_s$, we can conclude 
\begin{equation}
\begin{split}
    Pr[Precision(D_s) \geq pt] &\geq Pr[Precision(S) \geq pt] \geq prob \\
    \mathbb{E}[CR(D_s)] &\geq \mathbb{E}[CR(S)] \\
\end{split}
\end{equation}
\end{proof}

Lemma \ref{lemma:topk} supports the following theorem directly,

\begin{theorem}
The optimal solution to Problem \ref{problem:ptrt_w_assump} is a certain $\topkproxy{k}$ where $1 \leq k \leq |D|$.
\end{theorem}

Denote the optimal solution as $\topkproxy{k^*}$. Now, we are interested in how to find $D_{k^*}$ efficiently. In order to do that, we want to compare success probability and expected CR for any $\topkproxy{i}$ and $\topkproxy{j}$ where $1\leq i, j \leq |D|$. To achieve this, we have the following lemma,

\begin{lemma} [Monotonicity of Append]
\label{lemma:monoto_append}
Given $S \subseteq D$ of size $s$, $\gamma \in (0,1)$, and $p_j \in D \setminus S$.

(1)
\begin{equation}
\begin{split}
Pr[Recall(S) \geq \gamma] &\leq Pr[Recall(S\cup \{p_j\}) \geq \gamma]\\
\end{split}
\end{equation}

(2) When $\lceil s\gamma \rceil=\lceil (s+1)\gamma \rceil$,
\begin{equation}
\begin{split}
Pr[Precision(S) \geq \gamma] &\leq Pr[Precision(S\cup \{p_j\}) \geq \gamma]\\
\end{split}
\end{equation}
When $\lceil s\gamma \rceil+1=\lceil (s+1)\gamma \rceil$,
\begin{equation}
\begin{split}
Pr[Precision(S) \geq \gamma] &\geq Pr[Precision(S\cup \{p_j\}) \geq \gamma]\\
\end{split}
\end{equation}

\end{lemma}

\begin{proof}
Denote $S'= \{S \cup \{p_j\}\}$. We will first discuss precision, and then recall.

For precision, denote random variables $X=\sum_{p_i \in S} \mathbf{1}(p_i)$, and $Y=X+\mathbf{1}(p_j)$. Similarly, we can rewrite $Pr[Precision(S \cup \{p_j\})\geq \gamma]$ as $Pr[Y \geq \lceil (s+1)\gamma \rceil]$ and
\begin{equation}
\begin{split}
Pr[Y \geq \lceil (s+1)\gamma \rceil]
    &= \phi_j \cdot Pr[X=\lceil (s+1)\gamma \rceil-1] + Pr[X \geq \lceil (s+1)\gamma \rceil]
\end{split}
\end{equation}

When $\lceil s\gamma \rceil=\lceil (s+1)\gamma \rceil$, 
\begin{equation}
\end{equation}
\begin{equation}
\begin{split}
Pr[Y \geq \lceil (s+1)\gamma \rceil]
    &\geq Pr[X \geq \lceil (s+1)\gamma \rceil] = Pr[X \geq \lceil s\gamma \rceil]
\end{split}
\end{equation}

When $\lceil s\gamma \rceil+1=\lceil (s+1)\gamma \rceil$, 
\begin{equation}
\end{equation}
\begin{equation}
\begin{split}
Pr[Y \geq \lceil (s+1)\gamma \rceil]
    &\leq Pr[X = \lceil s\gamma \rceil] + Pr[X \geq \lceil s\gamma \rceil+1] = Pr[X \geq \lceil s\gamma \rceil]
\end{split}
\end{equation}
because $\phi_j \leq 1$.

Since $Pr[Precision(S)\geq \gamma]=Pr[X \geq \lceil s\gamma \rceil]$, the proof for precision is complete.

For recall, we are going to prove a stronger result, that is $Recall(S) \leq_{st} Recall(S')$. The proof is quite similar to the one to Lemma \ref{lemma:monoto_replace}, and here we only give a proof sketch.

When $\gamma = 0$, we have $Pr[Recall(S)\geq 0] = 1 \leq Pr[Recall(S')\geq 0] = 1$.

When $\gamma \in \mathbb{R} \setminus \{0\}$, denote $X_C=\sum_{p_i \in D \setminus S} \mathbf{1}(p_i)$, and $Y_C=X_C-\mathbf{1}(p_j)$. We can write
\begin{equation}
\begin{split}
    Pr[Recall(S) \geq \gamma] &= 
    \sum_{j=0}^{s} Pr[X=j]\cdot Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor],\\
    Pr[Recall(S') \geq \gamma] &=
    \sum_{j=0}^{s+1} Pr[Y=j]\cdot Pr[Y_C \leq \lfloor \frac{j}{\gamma} \rfloor].\\
\end{split}
\end{equation}

Next we can show 
\begin{equation}
\begin{split}
Pr[Y_C \leq \lfloor \frac{j}{\gamma} \rfloor]
    &= \phi_j \cdot Pr[X_C = \lfloor \frac{j}{\gamma} \rfloor+1] + Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor] \geq Pr[X_C \leq \lfloor \frac{j}{\gamma} \rfloor]
\end{split}
\end{equation}
By defining $\psi(x) := Pr[Y_C \leq \lfloor \frac{x}{\gamma} \rfloor]$, which is an increasing function, we can write the following inequality,
\begin{equation}
    Pr[Recall(S) \geq \gamma] \leq 
    \sum_{j=0}^{s} Pr[X=j]\cdot \psi(j) =\mathbb{E}[\psi(X)] .
\end{equation}
Since $X \leq_{st} Y$ \footnote{This result is easy to prove because $Y=X+\mathbf{1}(p_j)$, which suggests \textit{$Y$ is more likely than $X$ to take on large values}.}, by applying Proposition \ref{prop:st_expectation}, we have,
\begin{equation}
    Pr[Recall(S) \geq \gamma] \leq \mathbb{E}[\psi(X)] \leq \mathbb{E}[\psi(Y)] = Pr[Recall(S') \geq \gamma]
\end{equation}
for $\gamma \in \mathbb{R} \setminus \{0\}$. 

At last, we can conclude $Pr[Recall(S) \geq \gamma] \leq Pr[Recall(S') \geq \gamma]$ for $\gamma \in \mathbb{R}$ and therefore
\begin{equation}
    Recall(S) \leq_{st} Recall(S')
\end{equation}
\end{proof}

Similarly, we can have the monotonicity of expected recall for a given $S\subseteq D$,
\begin{lemma} [Monotonicity of Expectation (Append)]
\label{lemma:monoto_expect_append}
Given $S \subseteq D$ of size $s$, $\gamma \in (0,1)$, and $p_j \in D \setminus S$.
\begin{equation}
\begin{split}
\mathbb{E}[Recall(S)] \leq \mathbb{E}[Recall(S \cup \{p_j\})]
\end{split}
\end{equation}
\end{lemma}

\begin{proof}
Denote $S'=S \cup \{p_j\}$. Because $Recall(S) \leq_{st} Recall(S')$, by defining $\psi(x):=x$ and applying Proposition \ref{prop:st_expectation}, we have $\mathbb{E}[Recall(S)] \leq \mathbb{E}[Recall(S \cup \{p_j\})]$, same as the proof to Lemma \ref{lemma:monoto_expect_replace}.
\end{proof}

Lemma \ref{lemma:monoto_expect_append} says if we append new objects into an answer set, the expected recall will monotonically increase. Note expected recall is indeed $\mathbb{E}[CR]$ for PT-query, we can have the following theorem for PT-query under Assumption \ref{proxy_quality_assumption},

\begin{theorem} [PT-query With Quality Assumption]
\label{theorem:pt_second}
For a given PT-query, $D_{k^*} = D_{kmax}$ where $kmax = \max \{k \mid Pr[Precision(D_k) \geq pt] \geq prob\}$.
\end{theorem}

A native algorithm is to use linear search to compute $Pr[Precision(D_i) \geq pt]$ for $i=1,2,\cdots , |D|$ and return the largest $k$ ensuring high success probability. This naive algorithm, however, requires a full scan of the list $D_1, D_2, \cdots, D_{|D|}$, and could be expensive in practice.
It turns out that we can solve this problem by examining only a subset of $\{D_i \mid i=1,2,\cdots, |D|\}$, which gives us a more efficient algorithm. We will first introduce the algorithm for PT-query, and then RT-query.

For PT-query, we first use Lemma \ref{lemma:monoto_append} to identify all intervals $[ks, ke]$ where $Pr[Precision(D_i) \geq pt]$ monotonically increases or decreases on $i \in [ks, ke]$. Next, we compute $Pr[Precision(D_{ks}) \geq pt]$ and $Pr[Precision(D_{ke}) \geq pt]$ for all interval end points. We say an interval $[ks, ke]$ is \textit{proper} if either $Pr[Precision(D_{ks}) \geq pt] \geq prob$ or $Pr[Precision(D_{ke}) \geq pt] \geq prob$. 
We use $[ks^*, ke^*]$ to denote the proper interval of largest end point values. It is clear that $kmax \in [ks^*, ke^*]$. At last, we use a linear search to find $kmax$ on interval $[ks^*, ke^*]$. The algorithm is given as Algorithm \ref{alg:pt_query},

\begin{algorithm}
\caption{Algorithm for PT-query}
\label{alg:pt_query}
% \begin{algorithmic} [1]
% \Procedure{PT\_Query}{$D$, pt, prob}
% \State $intvl \gets [0]$; $probs \gets [1]$; $is\_incr \gets False$
% \For{$i \gets 1,2,\cdots , |D|$}
% \label{pt:comp_intvl_s}
% \If{($is\_incr$ \textbf{and} $\lceil i\cdot pt \rceil + 1 = \lceil (i+1)\cdot pt \rceil$) \textbf{or} (\textbf{not} $is\_incr$ \textbf{and} $\lceil i\cdot pt \rceil = \lceil (i+1)\cdot pt \rceil$) \textbf{or} $i=|D|$}
% \State $intvl.append(i)$
% \State $probs.append(\Call{PBPrecision}{D_i, pt})$
% \State $is\_incr \gets \neg is\_incr$
% \EndIf
% \EndFor
% \label{pt:comp_intvl_e}

% \State $proper\_intvl \gets [0,0]$
% \For{$i \gets 0, 1, \cdots,
% size(intvl)-1$}
% \label{pt:comp_proper_s}
% \If{$probs[i] \geq prob$ \textbf{or} $probs[i+1] \geq prob$}
% \State $proper\_intvl \gets [intvl[i], intvl[i+1]]$
% \EndIf
% \EndFor
% \label{pt:comp_proper_e}

% \State $k^* \gets argmax_k \{D_k \mid \Call{PBPrecision}{D_k, pt} \geq prob \land k \in proper\_intvl\}$
% \label{pt:comp_kmax}

% \State \Return $D_{k^*}$
% \EndProcedure
% \end{algorithmic}
\end{algorithm}

In line \ref{pt:comp_intvl_s} to \ref{pt:comp_intvl_e}, we construct a vector of all interval end points, $intvl$, by repeatedly applying Lemma \ref{lemma:monoto_append}. In line \ref{pt:comp_proper_s} to \ref{pt:comp_proper_e}, we compute the proper interval, $proper\_intvl$, of largest end points from $intvl$. In line \ref{pt:comp_kmax}, we use a linear search on $proper\_intvl$ to find $D_{kmax}$ which maximizes the expected recall rates according to our analysis. Algorithm \ref{alg:pt_query} invokes $PBPrecision$ for $O(|D|)$ objects and has an overall $O(|D|^3)$ time complexity.

For RT-query, because of Lemma \ref{lemma:monoto_append} and the fact $Recall(D)=1$, there exists a $k'$ where $Pr[Recall(D_k) \geq rt] \geq prob$ for $k' \leq k \leq |D|$. We first use a binary search to find $k'$. Next, we compute the $D_{k^*}$ which maximizes the expected precision through a linear search on the interval $[k', |D|]$. The algorithm is given in Algorithm \ref{alg:rt_query},

\begin{algorithm}
\caption{Algorithm for RT-query}
\label{alg:rt_query}
% \begin{algorithmic} [1]
% \Procedure{RT\_Query}{$D$, rt, prob}
% \State $L \gets 1$; $R \gets |D|$
% \label{rt:bs_s}
% \While {$L < R$}
% \State $mid \gets \lfloor (L + R) / 2 \rfloor$
% \If{$\Call{PBRecall}{D_{mid}, rt} < prob$}
% \State $L \gets mid+1$
% \Else
% \State $R \gets mid$
% \EndIf
% \EndWhile
% \label{rt:bs_e}

% \State $k^* \gets argmax_k\{\Call{ExpPrecision}{D_k} \mid k \in [L, |D|]\}$
% \label{rt:kstar}

% \State \Return $D_{k^*}$
% \EndProcedure
% \State
% \Procedure{ExpPrecision}{$D_k$}
% \State $PB \gets \Call{PBDistribution}{D_k}$
% \label{rt:exp_precis_s}
% \State $exp\_precis \gets \Call{Sum}{\frac{PB[1]\cdot 1}{k}, \frac{PB[2] \cdot 2}{k}, \cdots, \frac{PB[k] \cdot k}{k}}$

% \State \Return $exp\_precis$
% \label{rt:exp_precis_e}

% \EndProcedure
% \end{algorithmic}
\end{algorithm}

In line \ref{rt:bs_s} to \ref{rt:bs_e}, we use binary search to find the smallest $k=L$ which ensures the success probability of $D_L$ no less than $prob$, taking $O(log(|D|)|D|^2)$ time. In line \ref{rt:kstar}, we use linear search on the interval $[L, |D|]$ to find out the $D_{k^*}$ which maximizes the expected precision and return it as the answer. The computation of expected precision for the given $D_k$ is described in line \ref{rt:exp_precis_s} to \ref{rt:exp_precis_e}. We first compute the probability distribution $PB$ and then sums over the product between all possible precision outcomes and corresponding probabilities, which takes $O(|D|^2)$ time complexity. The overall running time is therefore dominated by the linear search (line \ref{rt:kstar}) and turns out to be $O(|D|^3)$. 

It is also worth to point out that, after the binary search (line \ref{rt:bs_s} to \ref{rt:bs_e}), we already figure out a group of valid answers (i.e., $D_{L}, D_{L+1}, \cdots, D_{|D|}$). If the application is sensitive to running time and tolerant to expected precision, we can run Algorithm \ref{alg:rt_query} as an anytime algorithm after completing line \ref{rt:bs_s} to \ref{rt:bs_e}.


\subsection{Algorithms with Known Query Selectivity - RT} \label{subsec:rt-algos}
We first show how to compute $Pr[ \sampleoptdepth{S} \geq \optdepth]$, for a given sample $S\subseteq D$, assuming the query selective is known, and derive the best sampling strategy accordingly.

\subsubsection{Computing $Pr[ \sampleoptdepth{S} \geq \optdepth]$}\hfill

Recall that $\optdepth = \min\{k|\frac{|\topkproxy{k}\cap A|}{|A|} \geq rt\}$, and $\sampleoptdepth{S} = \min\{k|S \cap A \subseteq \topkproxy{k}\}$. We have
\begin{equation}
\begin{split}
    Pr[ \sampleoptdepth{S} \geq \optdepth] &= Pr[\min\{k|S \cap A \subseteq \topkproxy{k}\} \geq \optdepth] \\
    &=1 - Pr[S \cap A \cap \{D \setminus \topkproxy{k^*-1}\} = \emptyset]
\end{split}
\end{equation}
In other words, $Pr[ \bar{i}_{S} \geq \bar{i}]$ equals to the probability that the given sample $S$ has a non-empty intersection with the set $A \cap \{p|\frac{|D_{\leq I(p)}\cap A|}{|A|} \geq rt\}$. The size of $A \cap \{I(p)|\frac{|D_{\leq I(p)}\cap A|}{|A|} \geq rt\}$ equals to $K=\lfloor |A|(1-rt)\rfloor+1$.

For a sample $S\subseteq D$ of size $s$,
\begin{equation}
Pr[S \cap A \cap \{p|\frac{|D_{\leq I(p)}\cap A|}{|A|} \geq rt\} \text{ is empty}] = \frac{\binom{|D|-K}{s}}{\binom{|D|}{s}}
\end{equation}

The success probability of a single draw can be written as 
\begin{equation}
\begin{split}
Pr[\bar{i}_{S} \geq \bar{i}] &= 1 - \frac{\binom{|D|-K}{s}}{\binom{|D|}{s}}\\
    &= 1 - \frac{(|D|-K)!(|D|-s)!}{(|D|)!(|D|-s-K)!}\\
    &= 1 - \prod_{i=0}^{K-1} \frac{|D|-s-i}{|D|-i}\\
    % &\geq 1 - (1-\frac{s}{|D|})^K\\
\end{split}
\end{equation}
where $K=\lfloor |A|(1-rt)\rfloor+1$.

\eat{
\begin{equation}
\begin{split}
\sum_{j=0}^{min\{|A|,s\}} Pr[\bar{i}_{S} \geq \bar{i} \mid  |S \cap A|=j] \cdot Pr[|S \cap A|=j]
\end{split}
\end{equation}


$Pr[|S \cap A|=j]$ is the probability that $S$ contains exactly $j$ qualified objects, which corresponds to a hypergeometric distribution \cite{babara2019stat}.

\begin{definition}
 [Hypergeometric Distribution]
Let the size of a finite population be $N$, with $K$ distinguished elements. \eat{belonging to Group $1$ and the other $N-K$ belonging to Group $2$.} Suppose we draw a sample of size $n$ without replacement, then the probability of seeing exactly $k$ distinguished elements is given by:
\begin{small}
\begin{equation}
\label{eq:pmf}
    pmf(k,N,K,n) = \frac{\binom{K}{k}\binom{N-K}{n-k}}{\binom{N}{n}}
\end{equation}
\end{small}
The survival function of seeing no less than $k$  distinct elements is: 
\begin{small}
\begin{equation}
\label{eq:svl}
    svl(k,N,K,n) = \sum_{i=k}^{min\{K, n\}} \frac{\binom{K}{i}\binom{N-K}{n-i}}{\binom{N}{n}}
\end{equation}
\end{small}
\end{definition}

From Eq. (\ref{eq:pmf}), we see that $Pr[|S \cap A|=j] = pmf(j,|D|,|A|,s)$. Furthermore, notice that objects in $A$ can be partitioned into $A_{<\bar{i}}$ and $A_{\geq \bar{i}}$ according to position values w.r.t. the index $I$. In a similar way, we can define $(S \cap A)_{<\bar{i}_{S}}$ and $(S \cap A)_{\geq \bar{i}_{S}}$. Since $\bar{i}$ and $\bar{i}_{S}$ respectively correspond to the smallest position in $A_{\geq \bar{i}}$ and $(S \cap A)_{\geq \bar{i}_{S}}$, we have $\bar{i} \leq \bar{i}_{S}$ if and only if $(S \cap A)_{\geq \bar{i}_{S}} \subseteq A_{\geq \bar{i}}$, which can be characterized by the survival function of a hypergeometric distribution with $N=|A|$, $K=|A_{\geq \bar{i}}|$, $n=|S \cap A|$, and $k=|(S \cap A)_{\geq \bar{i}_{S}}|$.
By definition, $|A_{\leq\bar{i}}| = \lceil rt \cdot |A| \rceil$, we have $|A_{\geq\bar{i}}|=|A_{>\bar{i}}|+1=|A|-|A_{\leq\bar{i}}|+1=\lfloor (1-rt) \cdot |A|\rfloor + 1$. Similarly, $|(S \cap A)_{\leq \bar{i}_{S}}| = \lceil rt \cdot |(S \cap A)| \rceil$ by definition, and we have $|(S \cap A)_{\geq \bar{i}_{S}}| = \lfloor (1-rt) \cdot |S \cap A| \rfloor + 1$, so

\begin{small}
\begin{equation}
\begin{split}
    Pr[\bar{i}_{S} \geq \bar{i} \mid |S \cap A|=j] &= svl(|(S \cap A)_{\geq \bar{i}_{S}}|, |A|, |A_{\geq \bar{i}}|, |S \cap A|)\\
    &= svl(\lfloor (1-rt) j \rfloor + 1, |A|, \lfloor (1-rt) |A|\rfloor + 1, j). \nonumber
\end{split}
\end{equation}
\end{small}

As a result, the success probability of a single draw is:
\begin{small}
\begin{equation}
\begin{split}
    Pr[\bar{i}_{S} \geq \bar{i}] &= \hspace*{-4ex} \sum_{j=0}^{min\{|A|,s\}} \hspace*{-3ex} pmf(j,|D|,|A|,s) \cdot svl(\lfloor (1-rt) j \rfloor + 1, |A|, \lfloor (1-rt) |A|\rfloor + 1, j) \nonumber %\\
    %&\triangleq f_{|A|}(s)
\end{split}
\end{equation}
\end{small}

Define $f_{|A|}(s) := Pr[\bar{i}_{S} \geq \bar{i}]$. 
}

Define $f_{|A|}(s) := Pr[\bar{i}_{S} \geq \bar{i}]$.
Notice that for a given dataset $D$, $f_{|A|}(s)$ is a function of $s$ parameterized by $|A|$. Let $\sigma$ be the query selectivity, we have $|A|=|D|\sigma$. 

Next, we want to derive the best sampling strategy based on this single draw success probability. We are going to discuss two cases: 1) where the exact value of $|A|$ is known; and 2) where a one-sided confidence interval $Pr[\alow \leq |A|] \geq 1-\delta$ is known. Later, we will show how to compute this kind of confidence interval in practice.

\eat{
Since $|A|$ is usually unknown beforehand, we need to estimate it by drawing extra samples. 
Let $\mathbf{1}_{cond}$ be an indicator function where $\mathbf{1}_{cond} = 1$ iff condition $cond$ holds.
For a randomly sampled object $p\in D$, the indicator value $\mathbf{1}_{p\in A}$ is a Bernoulli random variable with the expected value $\mathbb{E}[\mathbf{1}_{p\in A}]=\frac{|A|}{|D|}$. If we can obtain a good estimation of $\mathbb{E}[\mathbf{1}_{p\in A}]$, then we can compute $|A|$ directly as   $\mathbb{E}[\mathbf{1}_{p\in A}]\cdot |D|$. The most straightforward method is to draw $n$ singleton samples, $p_1, p_2, \cdots, p_n$, from $D$ with replacement and estimate\footnote{The function $\mathbf{1}_{p_i\in A}$ is evaluated using the oracle, for samples $p_i$.} $\mathbb{E}[\mathbf{1}_{p\in A}] \approx \frac{1}{n} \sum_{i=1}^n \mathbf{1}_{p_i\in A}$. Due to random variations in the sampling process, the estimation introduces new errors which can be propagated and affect the overall success probability. To control the estimation error, we employ Hoeffding bounds \cite{vershynin_2018} and compute the confidence intervals with the desired error rates.

\begin{proposition} [Hoeffding Bounds]\cite{vershynin_2018} 
Let $X_1, \cdots, X_n$ be i.i.d. Bernoulli random variables and let $Y = \frac{1}{n} \sum_{i=1}^n X_i$. Then for $\forall \epsilon \geq 0$, we have the one-sided  concentration bound
\begin{small}
\begin{equation}
\label{eq:oneside_hoeffding_bound}
    Pr[Y-\epsilon \leq \mathbb{E}[Y]] \geq 1-exp(-2n\epsilon^2)
\end{equation}
\end{small}
and the two-sided bound
\begin{small}
\begin{equation}
\label{eq:twoside_hoeffding_bound}
    Pr[Y-\epsilon \leq \mathbb{E}[Y] \leq Y+\epsilon] \geq 1-2exp(-2n\epsilon^2) 
\end{equation}
\end{small}
%where $exp(x) = e^x$.
\end{proposition}
Let $p_1, p_2, \cdots, p_n$, be independent singleton samples from $D$ with replacement. Define the indicator random variables $X_1, \cdots, X_{n}$, where $X_i = \mathbf{1}_{p_i\in A}$, $1 \leq i \leq n$. Let  $u$ denote the sampled query selectivity, that is, $u = \frac{1}{n}\sum_{i=1}^{n} X_i$. We can derive the confidence interval for the quantity $\frac{|A|}{|D|}$ as follows:
\begin{small}
\begin{equation}
\label{eq:ci_tpr}
    Pr[u - \epsilon \leq \frac{|A|}{|D|} \leq u + \epsilon]\geq 1-2exp(-2n\epsilon^2)
\end{equation}
\end{small}
\eat{ 
\note[Laks]{The above are bounds on the absolute error. Should we use bounds on the relative error instead?} 
\note[Dujian]{It will be great if we can. The challenge is that, the sample complexity of bounds on relative errors (e.g., Chernoff bounds) usually is a function of the interval width $\epsilon$ and the unknown mean $\mu$ (e.g., $\frac{|A|}{|D|}$ in our problem). As a result, one can derive an explicit sample complexity by manually constructing $\epsilon$ to eliminate the unknown variable $\mu$, in which sense the $\epsilon$ will then be a function of $\mu$. But in our case, we need both, that is, the explicit sample complexity and interval width $\epsilon$, where bounds on relative errors do not fit. }
} 
where $\epsilon \geq 0$. We further define $\aup := \lceil(u + \epsilon)|D|\rceil$ and $\alow := \lfloor(u - \epsilon)|D|\rfloor$ as the likely upper bound and lower bound for $|A|$. For any given $\delta$, we have $Pr[\alow \leq |A| \leq \aup] \geq 1-\delta$, provided $n \geq -\frac{log(\frac{\delta}{2})}{2\epsilon^2}$.

We are interested in $a_s \in [\alow, \aup]$ which gives the \textit{lowest} success probability for a single draw, i.e., $\forall a\colon \alow \leq a \leq \aup$, $f_{a}(s) \geq f_{a_s}(s)$. Interesting queries in real-world applications are usually selective. Since $a_s$ is an integer and the domain $[\alow, \aup]$ is bounded and is expected to be small, we can use brute force search to find the value of $a_s$ from $[\alow, \aup]$.  
\eat{In addition to the fact that $a_s$ is an integer, we can use brute-force search to find the exact value of $a_s$ from $[\alow, \aup]$.} In order to improve the efficiency, we further parallelize the computation of brute-force search and the average running time is within one second across our experiments, which is a fraction of \eat{the overall} a cost of invoking the oracle on the entire database \eat{we are interested in.}for our target applications.  
% \note[Laks]{Since this paper is about cost minimization, you need to say what is the cost of fnding $a_s$ by bruteforce? How does it compare with other costs such as optimization cost and oracle invocation cost.}
For a given sample $S$ of size $s$, we have $Pr[\bar{i}_S \geq \bar{i}] \geq f_{a_s}(s)$ with a probability no less than $1-\delta$, provided  $n \geq -\frac{log(\frac{\delta}{2})}{2\epsilon^2}$. Notice that $\delta$ and $\epsilon$ jointly control the sample  complexity of estimating $|A|$,\footnote{Equivalently, estimating query selectivity, for a given $D$.} which incurs extra oracle invocations. We want to choose $\delta$ and $\epsilon$, the sample size $s$ and the number of samples $m$ so as to \textit{minimize the overall cost}.
}

\subsubsection{Cost Minimization -- Given $|A|$}\hfill
\label{subsubsec:mincost_s_m}

Since applying the oracle to the whole dataset is prohibitively expensive, we are interested in the best $s$ and $m$, which result in minimal cost  and ensure high success probability. We define the cost as the number of oracle invocations, which equals the number of unique objects we see in the entire sampling process.
We can formalize the expected number of oracle invocations $N_{sample}$ for this repeated sampling phase as: 

\begin{small}
\begin{equation}
\label{eq:exp_cost_sample}
\begin{split} 
    \mathbb{E}[N_{sample}] = \mathbb{E}[|\bigcup_{i=1}^{m} S_i|]
    & = \mathbb{E}[\sum_{p \in D} \mathbf{1}_{p \in \bigcup_{i=1}^{m} S_i}] \\
    & = \sum_{p \in D} \mathbb{E}[\mathbf{1}_{p \in \bigcup_{i=1}^{m} S_i}] \\
    & = \sum_{p \in D} (1 - (1-\frac{s}{|D|})^{m}) \\
    & = |D|(1 - (1-\frac{s}{|D|})^{m})\\
\end{split}
\end{equation}
\end{small}
which is a function of $s, m$, denoted as $c(s,m)$.

Moreover, given $s$ and $m$, we have $ Pr[\bar{i}_{up} \geq \bar{i}] = Pr[\exists j\colon  1\leq j\leq m, \bar{i}_{S_j} \geq \bar{i}] = 1-(1-f_{|A|}(s))^{m}$.
\eat{If we know $\alow \leq |A| \leq \aup$, we can derive the lower bound for this conditional success probability as $Pr[\bar{i}_{up} \geq \bar{i} \mid \alow \leq |A| \leq \aup] \geq 1-(1-f_{a_s}(s))^{m}$.}

With the objective function (\ref{eq:exp_cost_sample}), we choose the best sampling strategy by solving the following optimization problem subject to a success probability constraint: 
\begin{equation}
\label{opt:samplesize_and_number}
\begin{split} 
     \textbf{minimize } c(s,m) &= |D|(1 - (1-\frac{s}{|D|})^{m})\\
    \textbf{s.t. } \\
    1-(1-f_{|A|}(s))^{m} &\geq prob   \\
\end{split}
\end{equation}

By plugging $f_{|A|}(s)=1 - \prod_{i=0}^{K-1} \frac{|D|-s-i}{|D|-i}$ into the constraint, we have 
\begin{equation}
    1-(1-f_{|A|}(s))^{m}=1-(\prod_{i=0}^{K-1} \frac{|D|-s-i}{|D|-i})^{m} \geq prob
\end{equation}
After swapping terms in both sides and take the logarithm, we get an equivalent constraint
\begin{equation}
    m \geq \frac{log(1-prob)}{log(\prod_{i=0}^{K-1} \frac{|D|-s-i}{|D|-i})}
\end{equation}
When $s$ is fixed, $c(s,m)$ monotonically increases when $m$ goes up. The smallest $m$ which ensures high success probability is therefore a function of $s$,

\begin{equation}
    m(s) = \lceil \frac{log(1-prob)}{log(\prod_{i=0}^{K-1} \frac{|D|-s-i}{|D|-i})} \rceil
\end{equation}

Given that, we can compute the corresponding $c(s,m(s))$ for each $1\leq s \leq |D|$, which takes $O(|D|^2)$ in total.

This exhaustive search algorithm can be inefficient in practice. We further offer an approximation algorithm which takes $O(|D|)$. The approximation algorithm fixes $s=1$ and computes $m(1)$ in $O(|D|)$ time. 
The approximation rate is defined as the ratio between saved cost $|D|-c(1,m(1))$ and the optimal saving $|D|-OPT$, where $OPT=\min_{s} \{c(s,m(s))\}$. We denote this ratio as $\gamma = \frac{|D|-c(1,m(1))}{|D|-OPT} \in (0, 1]$. Clearly, a larger $\gamma$ indicates a better cost saving and we would like to give a lower bound for $\gamma$.

First, we want to give a lower bound for $OPT$. Denote $\underline{m}(s)$ as
\begin{equation}
    \underline{m}(s) := \frac{log(1-prob)}{log(\prod_{i=0}^{K-1} \frac{|D|-s^*-i}{|D|-i})} \leq m(s).
\end{equation}
Because the cost increases when $m$ increases, we have $c(s,\underline{m(s)}) \leq c(s,m(s))$ and 
\begin{equation}
    \min_{s}\{ c(s,\underline{m}(s))\} \leq \min_{s} \{c(s,m(s))\} = OPT
\end{equation}
which is a lower bound for $OPT$.

Next, we want to compute $\min_{s}\{ c(s,\underline{m}(s))\}$. We have the following claim
\begin{claim}[Monotonicity of $c(s,\underline{m}(s))$]
Function $c(s,\underline{m}(s))$ monotonically decreases when $s > 0$.
\end{claim}
Since $1 \leq s \leq |D|-K$, we have $\min_{s}\{ c(s,\underline{m}(s))\} = c(D-K,\underline{m}(D-K))$. 

Now, we can give the approximation rate if we use $s=1$,
\begin{equation}
\begin{split}
\gamma = \frac{|D|-c(1,m(1))}{|D|-OPT} &\geq \frac{|D|-c(1,m(1))}{|D|-c(D-K,\underline{m}(D-K))} \\
&= \frac{(1-\frac{1}{|D|})^{\lceil \frac{log(1-prob)}{log(\prod_{i=0}^{K-1} \frac{|D|-1-i}{|D|-i})} \rceil}}{ (\frac{K}{|D|})^{ \frac{log(1-prob)}{log(\prod_{i=0}^{K-1} \frac{K-i}{|D|-i})} }} \\
&\geq \frac{(1-\frac{1}{|D|})^{ \frac{log(1-prob)}{log(\frac{|D|-K}{|D|})} + 1}}{(\frac{K}{|D|})^{ \frac{log(1-prob)}{\sum_{i=0}^{K-1}log(\frac{K-i}{|D|-i})} }} \\
\end{split}
\end{equation}

The expression is quite complicated, and we would like to simplify it. We first take logarithm on both sides,

\begin{equation}
\begin{split}
log(\gamma) &\geq log(1-\frac{1}{|D|}) -log(1-prob) \Big( \frac{log(1-\frac{1}{|D|})}{log(\frac{|D|}{|D|-K})} + \frac{log(\frac{|D|}{K})}{\sum_{i=0}^{K-1}log(\frac{|D|-i}{K-i})} \Big)\\
\end{split}
\end{equation}

We define $g(K) = \frac{log(1-\frac{1}{|D|})}{log(\frac{|D|}{|D|-K})}$ and $h(K) = \frac{log(\frac{|D|}{K})}{\sum_{i=0}^{K-1}log(\frac{|D|-i}{K-i})}$. Because $1-\frac{1}{x} \leq log(x) \leq x-1$ for $x>0$, we have
\begin{equation}
    g(K) \geq \frac{log(1-\frac{1}{|D|})}{1 - \frac{|D|-K}{|D|}} = \frac{log(1-\frac{1}{|D|})|D|}{K} 
    \geq -\frac{|D|}{K(|D|-1)}
\end{equation}
and
\begin{equation}
\begin{split}
 h(K) &\geq \frac{log(\frac{|D|}{K})}{\sum_{i=0}^{K-1}\frac{|D|-i}{K-i}-1}\\
 &=\frac{log(\frac{|D|}{K})}{(|D|-K)\sum_{i=1}^{K}\frac{1}{i}} \\
 &\geq \frac{\frac{|D|-K}{|D|}}{(|D|-K)K} \\
 &= \frac{1}{K|D|}
\end{split}
\end{equation}

By plugging these two lower bounds, we have
\begin{equation}
    log(\gamma) \geq log(1-\frac{1}{|D|}) -\frac{log(1-prob)}{K} \Big( \frac{1}{|D|} - \frac{|D|}{|D|-1}  \Big)
\end{equation}
After taking exponential, we have
\begin{equation}
    \gamma \geq (1-\frac{1}{|D|})(\frac{1}{1-prob})^{\frac{1}{K}( \frac{1}{|D|} - \frac{|D|}{|D|-1})}
\end{equation}
where $K=\lfloor |D|\sigma (1-rt)\rfloor+1$.
Denote this lower bound as $LB(|D|,prob,rt,\sigma)$.
We provide the following figures to help sense how good this lower bound could be in practice,
\begin{equation}
\begin{split}
LB(|D|=100000,prob=0.95,rt=0.95,\sigma=0.1)&=0.994\\
LB(|D|=100000,prob=0.99,rt=0.95,\sigma=0.1)&=0.991\\
LB(|D|=100000,prob=0.95,rt=0.99,\sigma=0.1)&=0.971\\
LB(|D|=100000,prob=0.95,rt=0.95,\sigma=0.01)&=0.943\\
\end{split}
\end{equation}

In general, we have the follow claim,
\begin{claim}
$LB(|D|,prob,rt,\sigma)$ decreases as $\sigma$ goes down or $rt$ goes up, and achieves the minima $(1-\frac{1}{|D|})(\frac{1}{1-prob})^{( \frac{1}{|D|} - \frac{|D|}{|D|-1})}$ when either $\sigma=0$ or $rt=1$. As $|D|$ goes to infinity, the minima converges to $1-prob$.
\end{claim}


\dujian{
\subsubsection{Cost Minimization -- Given $Pr[\alow \leq |A|] \geq 1-\delta$}\hfill
}
\dujian{
There are two new challenges, 1) the exact value of $|A|$ is unknown, instead we have a likely lower bound $\alow$; 2) the confidence interval brings new uncertainty which we should account for to ensure the overall success probability.}

\dujian{
For the first challenge, since $|A|$ is unknown, we can no longer use $f_{|A|}(s)$ as the lower bound for $Pr[\bar{i}_{S} \geq \bar{i}]$. We need a new lower bound, perhaps in a probabilistic way, and we are going to show $f_{\alow}(s)$ is the one we want. The idea is simple. Recall that $Pr[\bar{i}_{S} \geq \bar{i}] \geq 1 - (1-\frac{s}{|D|})^K$ where $K=\lfloor |A|(1-rt)\rfloor+1$. Denote $\underline{K}=\lfloor \alow(1-rt)\rfloor+1$, we have $Pr[\underline{K} \leq K] \geq 1-\delta$ because $Pr[\alow \leq |A|] \geq 1-\delta$. Then it can be easily examined that $Pr[Pr[\bar{i}_{S} \geq \bar{i}] \geq 1 - (1-\frac{s}{|D|})^{\underline{K}}] \geq 1-\delta$. And $f_{\alow}(s) = 1 - (1-\frac{s}{|D|})^{\underline{K}}$.}

\dujian{
For the second challenge, we need to use a more stringent probability threshold, $\hat{prob}$, to account for the new uncertainty. And the optimization problem is of the form,
\begin{equation}
\label{opt:samplesize_and_number}
\begin{split} 
     \textbf{minimize } cost_{prob} &= |D|(1 - (1-\frac{s}{|D|})^{m})\\
    \textbf{s.t. } \\
    1-(1-f_{\alow}(s))^{m} &\geq \hat{prob}   \\
\end{split}
\end{equation}
Since the error brought by the confidence interval of $|A|$ is independent with the sampling uncertainty, we have
\begin{equation} \label{eq: stat_guarantee}
\begin{split}
    Pr[\bar{i}_{up} \geq \bar{i}] &\geq Pr[\bar{i}_{up} \geq \bar{i} \land \alow \leq |A| ] \\
    &=Pr[\bar{i}_{up} \geq \bar{i} \mid \alow \leq |A|] \cdot Pr[\alow \leq |A|] \\
    &\geq \hat{prob} \cdot (1-\delta)\\
\end{split}
\end{equation}
Since we want $Pr[\bar{i}_{up} \geq \bar{i}] \geq prob$, $\hat{prob}$ is chosen to be at least $\frac{prob}{1-\delta}$. The optimization problem becomes
\begin{equation}
\label{opt:samplesize_and_number}
\begin{split} 
     \textbf{minimize } cost_{prob} &= |D|(1 - (1-\frac{s}{|D|})^{m})\\
    \textbf{s.t. } \\
    1-(1-f_{\alow}(s))^{m} &\geq \frac{prob}{1-\delta}   \\
\end{split}
\end{equation}
}

\hl{The optimality analysis is similar to  Problem (5), and will be added later.}


\eat{
where $\delta$ is the error rate of $|A|$ estimation and will be chosen later. That is, we will ensure the error rate is such that $Pr[\alow \leq |A| \leq \aup] \ge 1-\delta$. Also, since a small sample typically contains  few or even no qualified objects, we deliberately enforce a lower bound constraint on the sample size, $s \geq \frac{|D|}{\alow}$, to ensure that it  contains at least one qualified object with a high probability. 
%\note[Laks]{I don't see how it ensures that. E.g., if $\alow = |A|$, would choosing a singleton sample ensure that the sample drawn is a qualified object, in expectation? How?}
%\note[Dujian]{Good point, the lower bound for sample size is $s \geq \frac{|D|}{\alow}$ instead of $\frac{|A|}{\alow}$. A typo in writing.}


\begin{proposition}
Problem (\ref{opt:samplesize_and_number}) is non-convex.
\end{proposition}
\begin{proof}
Non-convexity of Problem (\ref{opt:samplesize_and_number}) is caused by the non-convex constraint $cons(s, m) = \frac{prob}{1-\delta} - 1 + (1-f_{a_s}(s))^{m} \leq 0$. The following counterexample shows the non-convexity of $cons(s, m)$. Without loss of generality,  assume $|A|$ is known and $a_s=|A|$. Given a setting where $|D|=10000$, $|A|=1000$, and $rt=0.9$, consider $s_1=100$, $s_2=400$, $m_1=m_2=1$, it can be easily shown that the interpolated point $0.9\cdot cons(s_1,m_1)+0.1\cdot cons(s_2,m_2) = 0.56$ is of a smaller value than $cons(0.9s_1+0.1s_2, 0.9m_1+0.1m_2)=0.57$. As a result, $cons(s,m)$ is not convex and so is Problem (\ref{opt:samplesize_and_number}).
\end{proof}

Problem (\ref{opt:samplesize_and_number}) is an instance of  a \textit{bi-level optimization} problem \cite{DBLP:journals/tec/SinhaMD18}. The upper-level problem asks for the best combination of $s$ and $m$, which relies on the value of $a_s$ returned by the lower-level problem. The lower-level problem aims to find $a_s$ in a given range $[\alow, \aup]$, and in turn requires $s$ as input. \eat{Such hierarchical optimization structure raises challenges of non-convexity and non-continuity, which make it difficult to be handled mathematically.} There are two challenges associated with Problem (\ref{opt:samplesize_and_number}): (i) the problem is neither convex nor continuous; (ii) there is mutual dependence between the two levels. 


To solve Problem (\ref{opt:samplesize_and_number}), we draw upon a body of methods known as clustering methods \cite{torn1986clustering}, which are designed for global optimization of problems whose objective functions are complex and expensive to evaluate. The intuition behind clustering methods, typically based on  \textit{Multistart}, is as follows: using a local optimization procedure \cite{kraft1988software}, repeatedly perform local search by sampling starting points.  However, a direct implementation of \textit{Multistart} may compute the same local optimum more than once yielding poor performance. Clustering methods were proposed to avoid such redundant computation. A typical clustering method consists of four steps \cite{torn1986clustering}:
\begin{enumerate}
    \item Sample points in the regions of interest;
    \item Transform samples to points grouped around local optimum;
    \item Use clustering methods to identify the groups (i.e., sub-domains containing local optimum);
    \item Perform local search on each sub-domain and return the best local optimum as the approximate global optimum.
\end{enumerate}
\begin{algorithm}
\caption{FindBestSampling()}
\label{alg:bilevel_opt_s_m}
\begin{small}
\begin{algorithmic}[1]
\Require problem parameters $param=(rt, prob, \delta, \epsilon, u)$
% \Require recall target $rt$, success probability $prob$;
% \Require parameter $\delta$ and $\epsilon$, query selectivity estimation $u$;
\Require lower-level optimizer $LOPT$, sample number $N$;
\State $s_u, m_u \gets \Call{Initialize}{ }$
\State $S \gets \Call{Sample}{\protect\Call{domainOf}{s,m}, size=N}$ \label{sm:sample}
\State $OBJ \gets \Call{ComputeObjective}{S, LOPT, param}$ \label{sm:objective}
\State $SD \gets \Call{FindSubdomain}{S,OBJ}$
\For{$sd \in SD$} \label{sm:cluster}
\State $local\_opt \gets \Call{LocalSearch}{sd, LOPT, param}$ \label{sm:localsearch}
\If{$local\_opt$ is better than $s_u, m_u$}
\State $s_u, m_u \gets local\_opt$
\EndIf
\EndFor
\State\Return $s_u, m_u$
\end{algorithmic}
\end{small}
\end{algorithm}

In the optimization process of Problem (\ref{opt:samplesize_and_number}), each sample is a pair  $(s,m)$ which instantiates a corresponding lower-level problem (see pseudo code is Algorithm \ref{alg:bilevel_opt_s_m}). Line \ref{sm:sample} draws $N$ samples from the variable domain of $s$ and $m$. Line \ref{sm:objective} computes the values of the objective function (\ref{eq:exp_cost_sample}) for each sample, while checking the constraint satisfaction of Problem (\ref{opt:samplesize_and_number}) with lower-level optimizer $LOPT$. In Line \ref{sm:cluster}, subdomains containing a local optimum are recognized with clustering  \cite{torn1986clustering} or by building a directed graph that connects samples to samples with a higher objective value \cite{torn1994tgo}. Each node with no incoming arcs indicates a local optimum neighborhood. Line \ref{sm:localsearch} uses a standard local search (e.g., SLSQP \cite{kraft1988software}) to compute the local optimum on each subdomain. The algorithm returns the best local optimum we found as $s_u$ and $m_u$.

Since the solution to the lower-level problem directly impacts our statistical guarantee,  we seek a sound approach to  return the optimal solution to that problem. 
Since the lower-level problem is discrete with a relatively small domain $|[\alow, \aup]|=2\epsilon|D|$, we employ a brute-force search on the bounded domain to solve it. $N$ is a hyper-parameter that controls how many samples to draw from the problem domains.  
We use a default value of $N=100$ in all our experiments and the optimization cost is observed to be seconds on average, which is a fraction of the cost of invoking the oracle on the entire database of interest.
% Intuitively, a large $N$ leads to a better quality of the approximated global optimum (i.e., expected overall sampling cost) but also a larger optimization cost. In Section \ref{sec:experiment}, we will demonstrate this trade-off through empirical results on real-world datasets and hint at possible strategies of setting the value of $N$ in practice. 

Since the lower-level optimizer is chosen to be sound and always return the exact $a_s$, 

We can show that the solution to Problem (\ref{opt:samplesize_and_number}) returned by \ours-RT satisfies the desired statistical guarantee.
\begin{theorem}
 [Statistical Guarantee of \ours-RT]
Given a recall-target query (Definition \ref{pt-rt-queries}), the success probability of \ours-RT is no less than the specified threshold, $prob$.
\end{theorem}
\begin{proof}
Let $s_u$, $m_u$ be the optimal choices given selectivity estimation $u$. We know the success probability of \ours-RT equals to $Pr[\bar{i}_{up} \geq \bar{i}]$, whose lower bound is given by

\begin{small}
\begin{equation} \label{eq: stat_guarantee}
\begin{split}
    Pr[\bar{i}_{up} \geq \bar{i}] &\geq Pr[\bar{i}_{up} \geq \bar{i} \land \alow \leq |A| \leq \aup] \\
    &=Pr[\bar{i}_{up} \geq \bar{i} \mid \alow \leq |A| \leq \aup] \cdot Pr[\alow \leq |A| \leq \aup] \\
    &\geq (1-(1-f_{a_s}(s_u))^{m_u}) \cdot (1-\delta)\\
    &\geq \frac{prob}{1-\delta} \cdot (1-\delta)\\
    &= prob
\end{split}
\end{equation}
\end{small}
\end{proof}
}

\subsubsection{Cost Minimization -- $\delta$, $\epsilon$}%\hfill
%Now, we need to choose $\delta$, and $\epsilon$ which were previously provided as parameters to Problem (\ref{opt:samplesize_and_number}). 
As can be seen from  Eq.  (\ref{eq:ci_tpr}), $\delta$ and $\epsilon$ control the sample complexity for estimating $|A|$, which  contributes  additional sampling cost. We want to determine $\delta$ and $\epsilon$ carefully to minimize the expected number of oracle invocations. %Following a similar procedure to derive objective (\ref{eq:exp_cost_sample}) 
Given $s$, $m$, and $n$, 
We can show that the expected overall sampling cost is: 
\begin{small}
\begin{equation}
\label{eq:exp_cost_overall}
\mathbb{E}[N_{overall}] = |D|(1-(1-\frac{s}{|D|})^{m}(1-\frac{1}{|D|})^{n})
\end{equation}
\end{small}
where $n$ is lower bounded by $-\frac{log(\frac{\delta}{2})}{2\epsilon^2}$. The choice of $s$ and $m$ relies on the sampled query selectivity $u$ estimated from the first $n$ draws,  which is a random variable. To make  objective (\ref{eq:exp_cost_overall}) computable, we need to expand the expected overall cost conditioned on the possibility of intermediate sampling results:
\begin{small}
\begin{equation} \label{eq:expected_total_cost}
\begin{split}
\mathbb{E}[N_{overall}] &= \mathbb{E}[\mathbb{E}[N_{overall} \mid u]]\\
&= \sum_{i = 0}^{n} \mathbb{E}[N_{overall} \mid u=\frac{i}{n}] \cdot Pr[u=\frac{i}{n}]    
\end{split}
\end{equation}
\end{small}
Specifically, by adopting the notation $s_u$ and $m_u$, we have: 
\begin{small}
\begin{equation}
\mathbb{E}[N_{overall} \mid u=\frac{i}{n}] = |D|(1-(1-\frac{s_u}{|D|})^{m_u}(1-\frac{1}{|D|})^{n})
\end{equation}
\end{small}
\begin{small}
\begin{equation}
Pr[u=\frac{i}{n}] = \sum_{j=1}^{|D|} Pr[u=\frac{i}{n} \mid |A|=j] \cdot Pr[|A|=j]
\end{equation}
\end{small}
\begin{small}
\begin{equation}
Pr[u=\frac{i}{n} \mid |A|=j] = \binom{n}{i} (\frac{j}{|D|})^{i} (1-\frac{j}{|D|})^{n - i}    
\end{equation}
\end{small}
following a binomial distribution. If we know the distribution of query selectivity (e.g., uniform), we can determine $Pr[|A|=j]$ and write:  
\begin{equation}
Pr[|A|=j] = \frac{1}{|D|}
\end{equation}
We can hence formulate the objective function as follows, which is further denoted as $cost_{total}$:
\begin{small}
\begin{equation} 
\begin{split}
\mathbb{E}[N_{overall}] &= \sum_{i = 0}^{n} \mathbb{E}[N_{overall} \mid u=\frac{i}{n}] \cdot Pr[u=\frac{i}{n}]\\
&= \sum_{i = 0}^{n} |D|(1-(1-\frac{s_u}{|D|})^{m_u}(1-\frac{1}{|D|})^{n})\\
&\ \times \sum_{j=1}^{|D|} \binom{n}{i} (\frac{j}{|D|})^{i} (1-\frac{j}{|D|})^{n - i} \cdot \frac{1}{|D|}
\end{split}
\end{equation}
\end{small}

The cost objective above relies on the uniform distribution assumption for query selectivity. It may however lead to poor performance when the true distribution significantly deviates from the assumption. For example, in real-world applications, queries are likely to be selective while the selectivity distribution may be complicated and hard to  model accurately. In light of this, we also propose an adaptive approach, which can choose parameters specific to the selectivity of the given query, through pilot sampling. More specifically, we will use a small sample (e.g., of 100 objects) to obtain a rough estimation $\hat{u}$ of query selectivity  and optimize the objective with respect to $\hat{u}$ ($0 < \delta, \epsilon < 1$): 
\begin{small}
\begin{equation} \label{opt:exp_cost_overall}
\begin{split}
\textbf{minimize }
cost_{total} &=  |D|(1-(1-\frac{s_{\hat{u}}}{|D|})^{m_{\hat{u}}}(1-\frac{1}{|D|})^{n}) \\
\textbf{s.t. } \\
    n &\geq -\frac{log(\frac{\delta}{2})}{2\epsilon^2}   \\
\end{split}
\end{equation}
\end{small}

Problem (\ref{opt:exp_cost_overall}) is built on Problem (\ref{opt:samplesize_and_number}) with additionally finding the best $\epsilon$ and $\delta$. This makes it a natural tri-level optimization problem. Given the problem complexity, we first reduce it to a bi-level version and  solve it with a clustering algorithm. The reduction is straightforward. Conceptually, the upper-level problem aims to find the best $\epsilon$ and $\delta$, which is dependent on the optimal expected cost. The lower-level problem outputs the optimal expected cost conditioned on each $\epsilon$ and $\delta$. The lower-level problem is similar to Problem (\ref{opt:samplesize_and_number}) whenever $\epsilon$ and $\delta$ are instantiated. 
Hence, we use Algorithm \ref{alg:bilevel_opt_s_m} with a modest modification for the lower-level optimizer, $LOPT$ (see Algorithm \ref{alg:bilevel_opt_delta_eps}). 
Line \ref{de:selectivity} draws a small sample of size $M$ from $D$ to estimate the query selectivity $\hat{u}$. Line \ref{de:sample} draws $N$ samples from the variable domain of $\delta$ and $\epsilon$. Line \ref{de:objective} computes the objective and constraint of Problem (\ref{opt:exp_cost_overall}) for each sample with the lower-level optimizer $LOPT$ and $\hat{u}$. 
The rest is similar to Algorithm \ref{alg:bilevel_opt_s_m}.
Lines \ref{de:subdomain}-\ref{de:enditr} identify neighborhoods where local optima are found by standard local search algorithms. The algorithm returns the best $\delta$ and $\epsilon$.
\begin{algorithm}
\caption{MinimizeOverallCost()}
\label{alg:bilevel_opt_delta_eps}
% \begin{small}
% \begin{algorithmic}[1]
% \Require problem parameters $param=(rt, prob)$;
% \Require lower-level optimizer $LOPT$, sample number $N$;
% \State $M \gets 100$
% \State $\hat{u} \gets \Call{EstimateQuerySelectivity}{D,size=M}$ \label{de:selectivity}
% \State $\delta, \epsilon \gets \Call{Initialize}{ }$
% \State $S \gets \Call{Sample}{\protect\Call{domainOf}{\delta,\epsilon}, size=N}$ \label{de:sample}
% \State $OBJ \gets \Call{ComputeObjective}{S, LOPT, param, \hat{u}}$ \label{de:objective}
% \State $SD \gets \Call{FindSubdomain}{S,OBJ}$ \label{de:subdomain}
% \For{$sd \in SD$}
% \State $local\_opt \gets \Call{LocalSearch}{sd, LOPT, param, \hat{u}}$ 
% \If{$local\_opt$ is better than $\delta, \epsilon$}
% \State $\delta, \epsilon \gets local\_opt$
% \EndIf
% \EndFor \label{de:enditr}
% \State\Return $\delta, \epsilon$
% \end{algorithmic}
% \end{small}
\end{algorithm}

Our overall algorithm, \ours-RT, depicted in Algorithm \ref{alg:our_rt}, is as follows.  We first compute the best $\delta, \epsilon$ by Algorithm \ref{alg:bilevel_opt_delta_eps}. Next, the query selectivity is estimated with Eq. (\ref{eq:ci_tpr}). Using $(\delta,\epsilon)$, and the selectivity estimate $u$, we derive the optimal $s_u$ and $m_u$ by Algorithm \ref{alg:bilevel_opt_s_m}. Finally, we draw $m_u$ samples of size $s_u$, $S_1, S_2, \cdots, S_{m_u}$, and compute $\bar{i}_{up} := max\{\bar{i}_{S_1}, \bar{i}_{S_2}, \cdots, \bar{i}_{S_{m_u}}\}$. The answer set is then returned as $Ans=D_{\bar{i}_{up}}$. Algorithm \ref{alg:our_rt} depicts our solution.


\begin{algorithm}
\caption{\ours-RT}
\label{alg:our_rt}
% \begin{algorithmic} [1]
% \Require problem parameters $param=(rt, prob)$;
% \State $\delta, \epsilon \gets \Call{MinimizeOverallCost}{param}$
% \State $n \gets \lceil -\frac{log(\frac{\delta}{2})}{2\epsilon^2} \rceil $
% \Comment{See Eq. (\ref{eq:ci_tpr})}
% \State $u \gets \Call{EsimateQuerySelectivity}{D,size=n}$
% \State $s_u, m_u \gets \Call{FindBestSampling}{param,\delta,\epsilon,u})$
% \For{$j \gets 1, 2, \cdots, m_u$}
% \State $S_j \gets \Call{Sample}{D, size=s_u}$
% \State $\bar{i}_{S_j} \gets $ the ($rt\cdot 100$)-percentile of $\{I(p)| p \in S_j \cap A\}$
% \EndFor
% \State $\bar{i}_{up} \gets max\{\bar{i}_{S_1}, \bar{i}_{S_2}, \cdots, \bar{i}_{S_{m_u}}\}$
% \State $Ans \gets \{p | p \in D \land I(p) \leq \bar{i}_{up}\}$
% \State \Return $Ans$
% \end{algorithmic}
\end{algorithm}
%The overall algorithm can be described as follows. We first compute a pair of $\delta$ and $\epsilon$ through pilot sampling and solving Problem (\ref{opt:exp_cost_overall}). Next, we derive the optimal $s_u$ and $m_u$ by estimating query selectivity with the given $\delta$ and $\epsilon$ and solving Problem (\ref{opt:samplesize_and_number}). Furthermore, we independently draw $m_u$ samples of size $s_u$, $S_1, S_2, \cdots, S_{m_u}$, and compute $\bar{i}_{up} = max\{\bar{i}_{S_1}, \bar{i}_{S_2}, \cdots, \bar{i}_{S_{m_u}}\}$. At the end, we return $Ans=D_{\leq \bar{i}_{up}}$ as the answer set.

% The pseudocode is given in Algorithm \ref{alg:our_rt}. 
% \begin{algorithm}
% \caption{Approximate Threshold-based Query with Recall-only Requirements}
% \label{alg:our_rt}
% \begin{algorithmic}
% \Require query object $q$, threshold $t$, recall target $rt$, success probability $prob$;
% \Require optimizer to problem (\ref{opt:exp_cost_overall}): $OPT_{\delta, \epsilon}$, optimizer to problem (\ref{opt:samplesize_and_number}): $OPT_{s,m}$;
% \State
% \State $M \gets 100$
% \State $\hat{u} \gets \Call{EstSelectivity}{D,size=M}$
% \State $\delta, \epsilon \gets OPT_{\delta, \epsilon}(D, rt, prob, \hat{u})$
% \State $n \gets \lceil -\frac{log(\frac{\delta}{2})}{2\epsilon^2} \rceil $
% \State $u \gets \Call{EstSelectivity}{D,size=n}$

% \State
% \State $s_u, m_u \gets OPT_{s,m}(D, u, \delta, \epsilon, prob, rt)$
% \For{$j \gets 1, 2, \cdots, m_u$}
% \State $S_j \gets \Call{Sample}{D, size=s_u}$
% \State $\bar{i}_{S_j} \gets $ the ($rt\cdot 100$)-percentile of $\{I(p)| p \in S_j \cap A\}$
% \EndFor
% \State $\bar{i}_{up} \gets max\{\bar{i}_{S_1}, \bar{i}_{S_2}, \cdots, \bar{i}_{S_{m_u}}\}$
% \State $Ans \gets \{p | p \in D \land I(p) \leq \bar{i}_{up}\} \cup \{p|p\in (\bigcup_{j=1}^{m_u} S_j) \cap A\}$
% \State
% \State \Return $Ans$
% \end{algorithmic}
% \end{algorithm}

% \note[Laks]{$\bar{i}_{S_i} \gets $ the ($rt\cdot 100$)-percentile of $\{I(p)| p \in S_i \cap A\}$. How do we compute this when we don't know $A$? Also, shouldn't $Ans$ also include all sampled objects which the oracle found to be  valid?}
% \note[Dujian]{For the first comment: we apply oracle on each sample $S_i$ which gives us $S_i \cap A$. For the second comment: yes, Ans does include all qualified objects found by sampling. }


\subsection{Algorithms for Precision-Target Queries}
\label{subsec:pt-algos}
\subsubsection{Phase 1: Pilot Sampling}\hfill
\label{subsubsec:phase_1}

An important observation is that, if chosen wisely, the proxy model should be able to emulate the oracle model. Given a query, qualified objects are expected to be located in the region of low positions $I(.)$, which implies the existence of dense regions including a majority of qualified objects and of reasonable recall rates. Since there may exist multiple dense regions, we want a union of them. Given a sample $S\subseteq D$, the problem can be formulated as follows:

\begin{problem} [FindLargestSubset]
Given a sample $S\subseteq D$ of size $s$, sort $p \in S$ by $I(p)$ increasingly as $p_1, p_2, \cdots, p_s$.
Denote $mean(i,j) = \frac{\sum_{k \in [i,j]} \mathbf{1}_{p_k \in A}}{j-i+1}$, where $\mathbf{1}_{p_k \in A}=1$ if $p_k$ is a qualified object; $\mathbf{1}_{p_k \in A}=0$, otherwise.
With a real number $c \in [0,1]$, we call an interval $[i,j]$ \textbf{proper} if $mean(i,j) \geq c$, and two intervals are \textbf{compatible} if they do not overlap. Let $G$ be the set of \textbf{proper} and mutually \textbf{compatible} intervals,
and further denote $\mathcal{G}$ as the set of all possible $G$. By defining $length(G) = \sum_{[i,j] \in G} j-i+1$, find $G_{max}$ where $\forall G \in \mathcal{G}$, $length(G) \leq length(G_{max})$. 
\end{problem}

With a sample $S$ of size $s$, a straightforward approach would first compute all $O(s^2)$ \textit{proper} intervals $[i,j]$,
and then sort them by the value of ending points, $j$, and starting points, $i$, in increasing order. Typically, proper intervals can be computed incrementally by $mean(i,j)=\frac{mean(i,j-1)\cdot (j-i) + \mathbf{1}_{p_j \in A}}{j-i+1}=\frac{mean(i+1,j)\cdot (j-i) + \mathbf{1}_{p_i \in A}}{j-i+1}$, and sorting can be done naturally along with this procedure. The time complexity is $O(s^2)$.
We use $opt[k]$ to track the optimal solution, $length(G_{max}^k)$, for a subset of proper intervals $[i,j]$ with $i \leq j \leq k$, $1\leq k \leq s$. We can compute the global optimum $opt[s]=length(G_{max})$ by dynamic programming, and the update rule is as follows,
\begin{small}
\begin{equation}
    opt[k] = max\{opt[k-1], max\{opt[i-1]+k-i+1 \mid [i,k] \text{ is proper}\}\}
\end{equation}
\end{small}
with $opt[0]=0$. We can also keep tracking of all intervals composing each $G_{max}^k$ along with the dynamic programming.
Since we only need to check all proper intervals once, the overall time complexity is $O(s^2)$.
Algorithm \ref{alg:find_dense_region} depicts our solution. 
\begin{algorithm}
\caption{$FindLargestSubset()$}
\label{alg:find_dense_region}
% \begin{small}
% \begin{algorithmic}[1]
% \Require dataset $D$, sample set $S$;
% \Require threshold $c$;

% \State $p_1,p_2,\cdots, p_s \gets \Call{Sort}{S, I(\cdot)}$
% \State $proper\_int \gets \Call{ComputeAndSortInterval}{p_1,p_2,\cdots, p_s, c}$
% \State $opt[0] \gets 0$
% \State $compos[0] \gets \emptyset$

% \For{$1 \leq k \leq s$}
% \State $proper\_int\_k \gets \Call{FetchIntervalEndBy\_K}{proper\_int}$
% \State $opt[k] \gets opt[k-1]$
% \State $compos[k] \gets compos[k-1]$
% \If{$proper\_int\_k$ is empty}
% \State \textbf{continue}
% \Else
% \ForAll{$[i,k] \in proper\_int\_k$}
% \If{$opt[i-1]+k-i+1 \geq opt[k]$}
% \State $opt[k] \gets opt[i-1]+k-i+1$
% \State $compos[k] \gets compos[i-1] \cup \{[i,k]\}$
% \EndIf
% \EndFor
% \EndIf
% \EndFor

% \State 
% \State $D' \gets \emptyset$
% \ForAll{$[i,j] \in compos[s]$}
% \State $D' \gets D' \cup D[I(p_i):I(p_j)]$
% \EndFor
% \State \Return $D'$
% \end{algorithmic}
% \end{small}
\end{algorithm}

\subsubsection{Phase 2: Iterative TPR Estimation}\hfill
\label{subsubsec:phase_2}

Given $D'$ (union of all plausible dense regions), we derive an answer set $Ans$ of high precision with a high probability. Following a sampling process as in Equation (\ref{eq:ci_tpr}), we estimate the TPR of $D'$ and denote the estimation as $u$. Given $\epsilon$, with the one-side Hoeffding bound in Equation (\ref{eq:oneside_hoeffding_bound}), we can derive a likely lower bound, $\tprlow{D'} = u-\epsilon$, for the true TPR of $D'$ with probability:
\begin{small}
\begin{equation}
\label{eq:tpr_lowerbound}
    Pr[u-\epsilon \leq \frac{|A\cap D'|}{|D'|}] \geq 1-exp(-2n\epsilon^2)
\end{equation}
\end{small}
where $n$ is the number of singleton samples. Given $\delta$, by enforcing $n \geq -\frac{log(\delta)}{2\epsilon^2}$, we can ensure $Pr[u-\epsilon \leq \frac{|A\cap D'|}{|D'|}] \geq 1-\delta$.
If $pt \leq u-\epsilon$ and $1-\delta \geq prob$, we can conclude $Pr[pt \leq \frac{|A\cap D'|}{|D'|}] \geq Pr[u-\epsilon \leq \frac{|A\cap D'|}{|D'|}] \geq prob$, and, therefore have $Ans=D'$.
However, it is possible that $pt \geq u-\epsilon$ due to a small value of $u$ or a large $\epsilon$. In this case, we can improve $u$ by purifying $D'$ with oracles, i.e., applying the oracle on a selected subset to filter out unqualified objects. Or, we can choose a more stringent $\epsilon$. The hope is that, with an improved $u$ and more stringent $\epsilon$, the refined lower bound exceeds $pt$ in the next round of estimation. 

Notice that, a stringent $\epsilon$ leads to a large number of samples required by the Hoeffding bound, and the purification of $D'$ also needs extra oracle invocations.
In light of this, we are interested in how to decide the value of $\epsilon$ and the number of oracle invocations for improving $u$, $N_{imp}$. It turns out that we can choose these two parameters jointly by solving the following optimization problem. Let $S \subseteq D'$ denote the selected subset for purification of size $N_{imp}$, the remained unexamined subset is $D'\setminus S$, from which we will draw samples to re-estimate the TPR.
The expected cost of purification and estimation is hence
\begin{small}
\begin{equation}
    cost_{pass} = N_{imp} + (|D'|-N_{imp})(1 - (1 -\frac{1}{|D'|-N_{imp}})^n)
\end{equation}
\end{small}
where $n$ is the number of singleton samples for estimation. Let $u'$ be the estimated TPR of $D' \setminus S$, and $u' - \epsilon$ be the corresponding lower bound. Since we memorize the qualified objects in purification, $S_{qual}$, we can always improve the lower bound by adding these qualified objects back to $D'\setminus S$. The lower bound, $\tprlow{D'}$, is improved to be
\begin{small}
\begin{equation}
\label{eq:tpr_lowerbound_refined}
\tprlow{D'} = \frac{(u' - \epsilon)(|D'|-N_{imp}) + |S_{qual}|}{|D'|-N_{imp}+|S_{qual}|}
\end{equation}
\end{small}
We want to choose $N_{imp}$ and $\epsilon$ by solving the following optimization problem,
\begin{small}
\begin{equation} \label{opt: find_eps_np}
\begin{split}
\textbf{minimize }
cost_{pass} &=  N_{imp} + (|D'|-N_{imp})(1 - (1 -\frac{1}{|D'|-N_{imp}})^n) \\
\textbf{s.t. } \\
    n &\geq -\frac{log(\delta)}{2\epsilon^2}    \\
    pt &\leq \tprlow{D'}
\end{split}
\end{equation}
\end{small}
where $0<\delta<1$. Because $u'$ is unknown beforehand, we use the plug-in estimate $u$ instead. We can show that Problem (\ref{opt: find_eps_np}) is non-convex.

\begin{proposition}
Problem (\ref{opt: find_eps_np}) is non-convex.
\end{proposition}
\begin{proof}
Non-convexity of Problem (\ref{opt: find_eps_np}) is caused by the non-convex constraint $cons(N_{imp},\epsilon) = pt - \tprlow{D'} \leq 0$. 
The following counterexample shows the non-convexity of $cons(N_{imp},\epsilon)$.
Given a setting where $|D'|=10000$, $pt=0.95$, $u'=0.96$, $|S_{qual}|=u'\cdot N_{imp}$, consider $N_{imp}^1=100$, $N_{imp}^2=900$, $\epsilon_1=0.01$, $\epsilon_2=0.1$. The interpolation point $0.5\cdot cons(N_{imp}^1,\epsilon_1) + 0.5\cdot cons(N_{imp}^2,\epsilon_2)=385$ is smaller than the middle point $cons(0.5(N_{imp}^1+N_{imp}^2), 0.5(\epsilon_1+\epsilon_2))=403$. As a result, $cons(N_{imp},\epsilon)$ is not convex and so is Problem (\ref{opt: find_eps_np}).
\end{proof}

We solve Problem (\ref{opt: find_eps_np}) with a clustering procedure similar to Algorithm \ref{alg:bilevel_opt_s_m} with the difference that we no longer need lower level optimization and the problem is solved on the domain of $\epsilon$ and $N_{imp}$.
Also, to overcome the extra error caused by the \textit{Multiple Hypothesis Testing} problem, we choose a stringent significance threshold in each iteration to be $\delta = \frac{1-prob}{\maxitr}$ and return the qualified objects discovered so far if no valid lower bound were found after $\maxitr$ iterations. Theorem \ref{thm:stat_pt} gives the statistical guarantee.

\begin{theorem}
 [Statistical Guarantee of \ours-PT]
 \label{thm:stat_pt}
Given a precision-target query (Definition \ref{pt-rt-queries}), the success probability of \ours-PT is no less than the specified threshold, $prob$.
\end{theorem}
\begin{proof}
Given $\maxitr$ and $\delta = \frac{1-prob}{\maxitr}$, denote $D'_i$ as the subset of interest at the $i$-th iteration, $term_i$ as a boolean vairable indicating if \ours-PT terminates at the $i$-th iteration, for $1\leq i \leq \maxitr$. Let $e$ be the overall error rate of \ours-PT, we are going to show $e \leq 1-prob$,
\begin{small}
\begin{equation} 
\begin{split}
    e &\leq \sum_{i=1}^{\maxitr} Pr[TPR(D'_i) < \tprlow{D'_i} \land term_i = True]\\
    & \leq \sum_{i=1}^{\maxitr} Pr[TPR(D'_i) < \tprlow{D'_i}]\\
    & = \sum_{i=1}^{\maxitr} (1-Pr[TPR(D'_i) \geq \tprlow{D'_i}])\\
    & \leq \maxitr \cdot \delta\\
    & = 1-prob
\end{split}
\end{equation}
\end{small}
\end{proof}
where the second last step is the direct application of Hoeffding bounds.
Algorithm \ref{alg:our_pt} depicts our solution.

\begin{algorithm}
\caption{\ours-PT}
\label{alg:our_pt}
% \begin{small}
% \begin{algorithmic} [1]
% \Require precision target $pt$, success probability $prob$;
% \Require $\maxitr \gets 5$; $M \gets 0.05\cdot |D|$; $S_{qual} \gets \emptyset$
% \State $\delta \gets \frac{1-prob}{\maxitr}$
% \State $S \gets \Call{Sample}{D, size=M}$
% \State $D' \gets \Call{FindLargestSubset}{D,S,c=pt}$
% \State $u \gets \frac{|S\cap D' \cap A|}{|S\cap D'|}$
% \Comment{Phase 1}
% \For{$i \gets 1,2,\cdots,\maxitr$}
% \State $\epsilon, N_{imp} \gets FindBestAllocation(D',pt,u,\delta)$
% \Comment{Solve Problem (\ref{opt: find_eps_np})}
% \State $S \gets Sample(D', size=N_{imp})$
% \State $S_{qual} \gets S_{qual} \cup (S \cap A)$
% \State $n \gets \lceil -\frac{log(\delta)}{2\epsilon^2} \rceil$
% \State $u \gets \Call{EstimateTPR}{D'\setminus S,size=n}$
% \If{$\frac{(u - \epsilon)(|D'|-N_{imp}) + |S_{qual}|}{|D'|-N_{imp}+|S_{qual}|} \geq pt$}
% \State \Return $Ans \gets (D'\setminus S) \cup S_{qual}$
% \Else
% \State $D' \gets D' \setminus S$
% \EndIf
% \EndFor
% \Comment{Phase 2}
% \State \Return $Ans \gets S_{qual} $
% \end{algorithmic}
% \end{small}
\end{algorithm}

}



==> free_writing.tex <==
yes

We utilize the fact that the proxy $\proxy$ is chosen as a simulator of the oracle $\oracle$. For any objects $p,q \in \Pi$, $\proxy(p)$ is expected to be a good approximation of $\oracle(p)$ and $dist(\proxy(p),\oracle(q))$ should be close to $dist(\oracle(p),\oracle(q))$. 

Given $q \in \Pi$, let $I_q(p): D \to \{1,2,\cdots, |D|\}$  be an index function, which returns an index value for each $p \in D$  in  increasing order of $dist(\proxy(p),\oracle(q))$. That is, if $p \in D$ is close to $q$ with respect to $\proxy(p)$ and $\oracle(q)$, then its index $I_q(p)$ should be a small value. We henceforth drop the subscript $q$ when the query $q$   is clear from the context.

Given a specific precision or recall target query, we expect the qualified objects to be clustered in the region of low indices $I(.)$. We expect that there exist dense regions of $I(.)$ that include a majority of qualified objects and enjoy a high true positive rate (TPR). By tightly estimating these dense regions with respect to either precision or recall targets, we can ensure that complementary rates are high. 

Let $D_{\leq i} = \{p | p \in D \land I(p) \leq i\}$ denote the subset of objects whose position is at most $i$ w.r.t. the index function $I(p)$.
For any given recall target $rt$, there always exists a \textit{minimal} position value $\bar{i}$ such that $\frac{|D_{\leq \bar{i}}\cap A|}{|A|} \geq rt$. 
For a position value $\bar{i}_{up}$, due to the monotonic relationship between $i$ and the recall rate of $D_{\leq i}$, we can safely return $Ans = D_{\leq \bar{i}_{up}}$ as the answer set, if we know that  $Pr[\bar{i}_{up} \geq \bar{i}] \geq prob$. We propose to use sampling to determine $\bar{i}_{up}$ and estimate $Pr[\bar{i}_{up} \geq \bar{i}]$.  

Similarly to $\bar{i}$, for each sample $S \subseteq D$, we define  $\bar{i}_{S}$   as the \textit{smallest} value for which $\frac{|D_{\leq \bar{i}_{S}}\cap A \cap S|}{|A \cap S|} \geq rt$;  each $\bar{i}_{S}$ corresponds to a success probability $Pr[\bar{i}_{S} \geq \bar{i}]$. 

{\bf Challenges.} The main idea for answering a recall-target query is to independently draw $m$ samples of size $s$, $S_1, S_2, \cdots, S_m$, \eat{and compute $\bar{i}_{up} = max\{\bar{i}_{S_1}, \bar{i}_{S_2}, \cdots, \bar{i}_{S_m}\}$} such that the probability $Pr[\bar{i}_{up} \geq \bar{i}] = 1 - \prod_{j=1}^{m}(1-Pr[\bar{i}_{S_j}\geq \bar{i}]) \geq prob$, where $\bar{i}_{up} := max\{\bar{i}_{S_1}, \bar{i}_{S_2}, \cdots, \bar{i}_{S_m}\}$.  This raises two challenges: (1) how to compute the probability $Pr[ \bar{i}_{S} \geq \bar{i}]$ for a given sample $S$? and  (2) given that the oracle invocation is expensive, how to sample such that the number of oracle invocations is minimized, while ensuring a success probability no less than $prob$? 

{\bf Solution Overview.} Our solution, \ours-RT, is depicted in Figure \ref{fig:our_rt} (details and algorithms   in \S \ref{subsec:rt-algos}). We leverage the observation that for a given sample $S$, the probability $Pr[\bar{i}_{S} \geq \bar{i}]$ corresponds to a hypergeometric distribution \cite{babara2019stat} parameterized by $|A|$. The best sampling strategy (i.e., sample size $s$ and number of samples $m$) depends on the query selectivity $\frac{|A|}{|D|}$ and can be derived by solving an optimization problem that ensures $prob$ and minimizes the expected sampling cost, $cost_{prob}$. Since query selectivity is  unknown beforehand, we  estimate it through another round of sampling with concentration bounds (i.e., Hoeffding bounds \cite{vershynin_2018}), which is further controlled parameters $\delta$ and $\epsilon$. This leads to more oracle invocations in addition to $cost_{prob}$, so we want to choose $\delta$ and $\epsilon$ so as to minimizing the expected total sampling cost, $cost_{total}$. 
